An Eager Splitting Strategy for Online Decision Trees

Decision tree ensembles are widely used in practice. In this work, we study in ensemble settings the effectiveness of replacing the split strategy for the state-of-the-art online tree learner, Hoeffding Tree, with a rigorous but more eager splitting strategy that we had previously published as Hoeffding AnyTime Tree. Hoeffding AnyTime Tree (HATT), uses the Hoeffding Test to determine whether the current best candidate split is superior to the current split, with the possibility of revision, while Hoeffding Tree aims to determine whether the top candidate is better than the second best and if a test is selected, fixes it for all posterity. HATT converges to the ideal batch tree while Hoeffding Tree does not. We find that HATT is an efficacious base learner for online bagging and online boosting ensembles. On UCI and synthetic streams, HATT as a base learner outperforms HT within a 0.05 significance level for the majority of tested ensembles on what we believe is the largest and most comprehensive set of testbenches in the online learning literature. Our results indicate that HATT is a superior alternative to Hoeffding Tree in a large number of ensemble settings.

==> menrsyn2.tex <==
-s (RecurrentConceptDriftStream -x 200000 -y 200000 -z 100 -s (generators.AgrawalGenerator -f 2 -i 2) -d (generators.AgrawalGenerator -f 3 -i 3)) & \textbf{0.11929} & 0.13103 \\
-s (RecurrentConceptDriftStream -x 200000 -y 200000 -z 100 -s (generators.RandomTreeGenerator -r 1 -i 1) -d (generators.RandomTreeGenerator -r 2 -i 2)) & 0.09511 & \textbf{0.08372} \\
-s (RecurrentConceptDriftStream -x 200000 -y 200000 -z 100 -s (generators.SEAGenerator -f 2 -i 2) -d (generators.SEAGenerator -f 3 -i 3)) & 0.11452 & \textbf{0.11273} \\
-s (RecurrentConceptDriftStream -x 200000 -y 200000 -z 100 -s (generators.STAGGERGenerator -i 2 -f 2) -d (generators.STAGGERGenerator -i 3 -f 3)) & \textbf{0.00172} & 0.00301 \\
-s (generators.HyperplaneGenerator -k 10 -t 0.0001 -i 2) & \textbf{0.10114} & 0.10417 \\
-s (generators.HyperplaneGenerator -k 10 -t 0.01 -i 2) & \textbf{0.11091} & 0.11577 \\
-s (generators.HyperplaneGenerator -k 5 -t 0.0001 -i 2) & \textbf{0.09972} & 0.10192 \\
-s (generators.HyperplaneGenerator -k 5 -t 0.01 -i 2) & \textbf{0.10014} & 0.10313 \\
-s (generators.LEDGeneratorDrift -d 1 -i 2) & \textbf{0.25996} & 0.26016 \\
-s (generators.RandomRBFGeneratorDrift -s 0.0001 -k 10 -i 2 -r 2) & 0.07738 & \textbf{0.07149} \\
-s (generators.RandomRBFGeneratorDrift -s 0.0001 -k 50 -i 2 -r 2) & 0.13282 & \textbf{0.11325} \\
-s (generators.RandomRBFGeneratorDrift -s 0.001 -k 10 -i 2 -r 2) & 0.11143 & \textbf{0.10667} \\
-s (generators.RandomRBFGeneratorDrift -s 0.001 -k 50 -i 2 -r 2) & 0.30834 & \textbf{0.29937} \\
-s (generators.WaveformGeneratorDrift -d 1 -i 2 -n) & 0.14594 & \textbf{0.14317} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 2 -n 2 -v 2 -r 2 -b 200000 -d Recurrent) & 0.12285 & \textbf{0.11331} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 2 -v 2 -r 2 -b 200000 -d Recurrent) & 0.16658 & \textbf{0.15409} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 3 -v 2 -r 2 -b 200000 -d Recurrent) & \textbf{0.11804} & 0.12085 \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 3 -v 3 -r 2 -b 200000 -d Recurrent) & \textbf{0.14935} & 0.16353 \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 3 -v 4 -r 2 -b 200000 -d Recurrent) & \textbf{0.1531} & 0.22027 \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 3 -v 5 -r 2 -b 200000 -d Recurrent) & \textbf{0.18661} & 0.20877 \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 4 -n 2 -v 2 -r 2 -b 200000 -d Recurrent) & \textbf{0.12408} & 0.12903 \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 4 -n 4 -v 4 -r 2 -b 200000 -d Recurrent) & \textbf{0.17194} & 0.21027 \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 5 -n 2 -v 2 -r 2 -b 200000 -d Recurrent) & \textbf{0.11097} & 0.11112 \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 5 -n 5 -v 5 -r 2 -b 200000 -d Recurrent) & 0.29009 & \textbf{0.18} \\
\bottomrule &  &  \\
\begin{tabularx}{\linewidth}{Xr}
		A \textbf{bold} value indicates higher accuracy, and \textit{\textbf{bold italics}} indicate a tie.  & \textbf{Unique Wins}
		\end{tabularx} & \textbf{14} & \textbf{10} \\
\cmidrule[0.4pt](lr){2-3} &  &  \\
\begin{tabularx}{\linewidth}{Xr} The test is a one-tailed binomial test to determine the probability that the strategy in the rightmost column would achieve so many wins if wins and losses were equiprobable. & \textbf{Test Statistics} \end{tabularx} & \textbf{p-value: 0.84627} & \textbf{Confidence Interval:  0.24639 --- 1} \\


==> menrsyn3.tex <==
-s (RecurrentConceptDriftStream -x 200000 -y 200000 -z 100 -s (generators.AgrawalGenerator -f 2 -i 2) -d (generators.AgrawalGenerator -f 3 -i 3)) & 0.11408 & \textbf{0.11073} \\
-s (RecurrentConceptDriftStream -x 200000 -y 200000 -z 100 -s (generators.RandomTreeGenerator -r 1 -i 1) -d (generators.RandomTreeGenerator -r 2 -i 2)) & 0.06448 & \textbf{0.06214} \\
-s (RecurrentConceptDriftStream -x 200000 -y 200000 -z 100 -s (generators.SEAGenerator -f 2 -i 2) -d (generators.SEAGenerator -f 3 -i 3)) & 0.10672 & \textbf{0.10636} \\
-s (RecurrentConceptDriftStream -x 200000 -y 200000 -z 100 -s (generators.STAGGERGenerator -i 2 -f 2) -d (generators.STAGGERGenerator -i 3 -f 3)) & \textbf{0.00137} & 0.00142 \\
-s (generators.HyperplaneGenerator -k 10 -t 0.0001 -i 2) & \textbf{0.10714} & 0.10864 \\
-s (generators.HyperplaneGenerator -k 10 -t 0.01 -i 2) & \textbf{0.11623} & 0.1187 \\
-s (generators.HyperplaneGenerator -k 5 -t 0.0001 -i 2) & \textbf{0.10488} & 0.10579 \\
-s (generators.HyperplaneGenerator -k 5 -t 0.01 -i 2) & \textbf{0.09741} & 0.0986 \\
-s (generators.LEDGeneratorDrift -d 1 -i 2) & \textbf{0.26033} & 0.27963 \\
-s (generators.RandomRBFGeneratorDrift -s 0.0001 -k 10 -i 2 -r 2) & 0.0605 & \textbf{0.05854} \\
-s (generators.RandomRBFGeneratorDrift -s 0.0001 -k 50 -i 2 -r 2) & 0.08728 & \textbf{0.08558} \\
-s (generators.RandomRBFGeneratorDrift -s 0.001 -k 10 -i 2 -r 2) & 0.08917 & \textbf{0.08612} \\
-s (generators.RandomRBFGeneratorDrift -s 0.001 -k 50 -i 2 -r 2) & 0.18823 & \textbf{0.1742} \\
-s (generators.WaveformGeneratorDrift -d 1 -i 2 -n) & 0.14674 & \textbf{0.14573} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 2 -n 2 -v 2 -r 2 -b 200000 -d Recurrent) & \textbf{0.08568} & 0.09068 \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 2 -v 2 -r 2 -b 200000 -d Recurrent) & 0.15231 & \textbf{0.15097} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 3 -v 2 -r 2 -b 200000 -d Recurrent) & \textbf{0.11588} & 0.1206 \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 3 -v 3 -r 2 -b 200000 -d Recurrent) & \textbf{0.15151} & 0.15941 \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 3 -v 4 -r 2 -b 200000 -d Recurrent) & \textbf{0.21071} & 0.22021 \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 3 -v 5 -r 2 -b 200000 -d Recurrent) & \textbf{0.20627} & 0.21383 \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 4 -n 2 -v 2 -r 2 -b 200000 -d Recurrent) & 0.10922 & \textbf{0.10595} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 4 -n 4 -v 4 -r 2 -b 200000 -d Recurrent) & \textbf{0.17353} & 0.21386 \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 5 -n 2 -v 2 -r 2 -b 200000 -d Recurrent) & \textbf{0.11904} & 0.12773 \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 5 -n 5 -v 5 -r 2 -b 200000 -d Recurrent) & \textbf{0.13153} & 0.17235 \\
\bottomrule &  &  \\
\begin{tabularx}{\linewidth}{Xr}
		A \textbf{bold} value indicates higher accuracy, and \textit{\textbf{bold italics}} indicate a tie.  & \textbf{Unique Wins}
		\end{tabularx} & \textbf{14} & \textbf{10} \\
\cmidrule[0.4pt](lr){2-3} &  &  \\
\begin{tabularx}{\linewidth}{Xr} The test is a one-tailed binomial test to determine the probability that the strategy in the rightmost column would achieve so many wins if wins and losses were equiprobable. & \textbf{Test Statistics} \end{tabularx} & \textbf{p-value: 0.84627} & \textbf{Confidence Interval:  0.24639 --- 1} \\


==> mev1.tex <==
 RecurrentConceptDriftStream -x 200000 -y 200000 -z 100  AgrawalGenerator -f 2 -i 2 -d AgrawalGenerator -f 3 -i 3 & \textbf{011073} & 01739 \\
 RecurrentConceptDriftStream -x 200000 -y 200000 -z 100  RandomTreeGenerator -r 1 -i 1 -d RandomTreeGenerator -r 2 -i 2 & \textbf{006214} & 018482 \\
 RecurrentConceptDriftStream -x 200000 -y 200000 -z 100  SEAGenerator -f 2 -i 2 -d SEAGenerator -f 3 -i 3 & \textbf{010636} & 013493 \\
 RecurrentConceptDriftStream -x 200000 -y 200000 -z 100  STAGGERGenerator -i 2 -f 2 -d STAGGERGenerator -i 3 -f 3 & \textbf{000142} & 01926 \\
 HyperplaneGenerator -k 10 -t 00001 -i 2 & \textbf{010864} & 011174 \\
 HyperplaneGenerator -k 10 -t 0001 -i 2 & \textbf{011789} & 01276 \\
 HyperplaneGenerator -k 10 -t 001 -i 2 & \textbf{01187} & 012948 \\
 HyperplaneGenerator -k 5 -t 00001 -i 2 & \textbf{010579} & 010955 \\
 HyperplaneGenerator -k 5 -t 0001 -i 2 & \textbf{010984} & 012183 \\
 HyperplaneGenerator -k 5 -t 001 -i 2 & \textbf{00986} & 011885 \\
 LEDGeneratorDrift -d 1 -i 2 & 027963 & \textbf{026022} \\
 LEDGeneratorDrift -d 3 -i 2 & 027944 & \textbf{026022} \\
 LEDGeneratorDrift -d 5 -i 2 & 02796 & \textbf{026022} \\
 LEDGeneratorDrift -d 7 -i 2 & 027973 & \textbf{026022} \\
 RandomRBFGeneratorDrift  00001 -k 10 -i 2 -r 2 & \textbf{005854} & 006263 \\
 RandomRBFGeneratorDrift  00001 -k 50 -i 2 -r 2 & \textbf{008558} & 011581 \\
 RandomRBFGeneratorDrift  0001 -k 10 -i 2 -r 2 & \textbf{008612} & 009147 \\
 RandomRBFGeneratorDrift  0001 -k 50 -i 2 -r 2 & \textbf{01742} & 029518 \\
 WaveformGeneratorDrift -d 1 -i 2 -n & \textbf{014573} & 014887 \\
 WaveformGeneratorDrift -d 3 -i 2 -n & \textbf{014574} & 014887 \\
 WaveformGeneratorDrift -d 5 -i 2 -n & \textbf{014574} & 014886 \\
 WaveformGeneratorDrift -d 7 -i 2 -n & \textbf{014574} & 014886 \\
 AbruptDriftGenerator -c  -o 10 -z 2 -n 2 -v 2 -r 2 -b 200000 -d Recurrent & \textbf{009068} & 03104 \\
 AbruptDriftGenerator -c  -o 10 -z 3 -n 2 -v 2 -r 2 -b 200000 -d Recurrent & \textbf{015097} & 036394 \\
 AbruptDriftGenerator -c  -o 10 -z 3 -n 3 -v 2 -r 2 -b 200000 -d Recurrent & \textbf{01206} & 032268 \\
 AbruptDriftGenerator -c  -o 10 -z 3 -n 3 -v 3 -r 2 -b 200000 -d Recurrent & \textbf{015941} & 035155 \\
 AbruptDriftGenerator -c  -o 10 -z 3 -n 3 -v 4 -r 2 -b 200000 -d Recurrent & \textbf{022021} & 037892 \\
 AbruptDriftGenerator -c  -o 10 -z 3 -n 3 -v 5 -r 2 -b 200000 -d Recurrent & \textbf{021383} & 037639 \\
 AbruptDriftGenerator -c  -o 10 -z 4 -n 2 -v 2 -r 2 -b 200000 -d Recurrent & \textbf{010595} & 032019 \\
 AbruptDriftGenerator -c  -o 10 -z 4 -n 4 -v 4 -r 2 -b 200000 -d Recurrent & \textbf{021386} & 037445 \\
 AbruptDriftGenerator -c  -o 10 -z 5 -n 2 -v 2 -r 2 -b 200000 -d Recurrent & \textbf{012773} & 033627 \\
 AbruptDriftGenerator -c  -o 10 -z 5 -n 5 -v 5 -r 2 -b 200000 -d Recurrent & \textbf{017235} & 034243 \\
\bottomrule &  &  \\
\begin{tabularx}{\linewidth}{Xr}
		A \textbf{bold} value indicates higher accuracy, and \textit{\textbf{bold italics}} indicate a tie  & \textbf{Unique Wins}
		\end{tabularx} & \textbf{28} & \textbf{4} \\
\cmidrule[04pt]lr{2-3} &  &  \\
\begin{tabularx}{\linewidth}{Xr} The test is a one-tailed binomial test to determine probability that the strategy in the  
             column is likely to have lower accuracy in more than half of the experiments & \textbf{Test Statistics} \end{tabularx} & \textbf{p-value: 1} & \textbf{Confidence Interval:  004385 --- 1} \\


==> mev10.tex <==
 RecurrentConceptDriftStream -x 200000 -y 200000 -z 100  AgrawalGenerator -f 2 -i 2 -d AgrawalGenerator -f 3 -i 3 & 02859 & \textbf{017972} \\
 RecurrentConceptDriftStream -x 200000 -y 200000 -z 100  RandomTreeGenerator -r 1 -i 1 -d RandomTreeGenerator -r 2 -i 2 & 02768 & \textbf{024893} \\
 RecurrentConceptDriftStream -x 200000 -y 200000 -z 100  SEAGenerator -f 2 -i 2 -d SEAGenerator -f 3 -i 3 & 011277 & \textbf{011094} \\
 RecurrentConceptDriftStream -x 200000 -y 200000 -z 100  STAGGERGenerator -i 2 -f 2 -d STAGGERGenerator -i 3 -f 3 & \textbf{000114} & 000115 \\
 HyperplaneGenerator -k 10 -t 00001 -i 2 & 018103 & \textbf{017801} \\
 HyperplaneGenerator -k 10 -t 0001 -i 2 & 017637 & \textbf{017286} \\
 HyperplaneGenerator -k 10 -t 001 -i 2 & 017949 & \textbf{017439} \\
 HyperplaneGenerator -k 5 -t 00001 -i 2 & 018979 & \textbf{018213} \\
 HyperplaneGenerator -k 5 -t 0001 -i 2 & 019797 & \textbf{0163} \\
 HyperplaneGenerator -k 5 -t 001 -i 2 & 020885 & \textbf{015292} \\
 LEDGeneratorDrift -d 1 -i 2 & 03201 & \textbf{029301} \\
 LEDGeneratorDrift -d 3 -i 2 & 04301 & \textbf{03153} \\
 LEDGeneratorDrift -d 5 -i 2 & 056805 & \textbf{028743} \\
 LEDGeneratorDrift -d 7 -i 2 & 059338 & \textbf{027797} \\
 RandomRBFGeneratorDrift  00001 -k 10 -i 2 -r 2 & 021325 & \textbf{01804} \\
 RandomRBFGeneratorDrift  00001 -k 50 -i 2 -r 2 & 019752 & \textbf{016872} \\
 RandomRBFGeneratorDrift  0001 -k 10 -i 2 -r 2 & 020761 & \textbf{018411} \\
 RandomRBFGeneratorDrift  0001 -k 50 -i 2 -r 2 & 025834 & \textbf{02469} \\
 WaveformGeneratorDrift -d 1 -i 2 -n & 025626 & \textbf{019998} \\
 WaveformGeneratorDrift -d 3 -i 2 -n & 025283 & \textbf{019722} \\
 WaveformGeneratorDrift -d 5 -i 2 -n & 025061 & \textbf{019728} \\
 WaveformGeneratorDrift -d 7 -i 2 -n & 02301 & \textbf{019369} \\
 AbruptDriftGenerator -c  -o 10 -z 2 -n 2 -v 2 -r 2 -b 200000 -d Recurrent & 008701 & \textbf{000892} \\
 AbruptDriftGenerator -c  -o 10 -z 3 -n 2 -v 2 -r 2 -b 200000 -d Recurrent & 003985 & \textbf{001944} \\
 AbruptDriftGenerator -c  -o 10 -z 3 -n 3 -v 2 -r 2 -b 200000 -d Recurrent & \textbf{002768} & 003412 \\
 AbruptDriftGenerator -c  -o 10 -z 3 -n 3 -v 3 -r 2 -b 200000 -d Recurrent & 00731 & \textbf{002412} \\
 AbruptDriftGenerator -c  -o 10 -z 3 -n 3 -v 4 -r 2 -b 200000 -d Recurrent & 012644 & \textbf{004636} \\
 AbruptDriftGenerator -c  -o 10 -z 3 -n 3 -v 5 -r 2 -b 200000 -d Recurrent & 016281 & \textbf{004863} \\
 AbruptDriftGenerator -c  -o 10 -z 4 -n 2 -v 2 -r 2 -b 200000 -d Recurrent & 005672 & \textbf{001634} \\
 AbruptDriftGenerator -c  -o 10 -z 4 -n 4 -v 4 -r 2 -b 200000 -d Recurrent & 041422 & \textbf{018882} \\
 AbruptDriftGenerator -c  -o 10 -z 5 -n 2 -v 2 -r 2 -b 200000 -d Recurrent & 003036 & \textbf{001805} \\
 AbruptDriftGenerator -c  -o 10 -z 5 -n 5 -v 5 -r 2 -b 200000 -d Recurrent & 070713 & \textbf{054099} \\
\bottomrule &  &  \\
\begin{tabularx}{\linewidth}{Xr}
		A \textbf{bold} value indicates higher accuracy, and \textit{\textbf{bold italics}} indicate a tie  & \textbf{Unique Wins}
		\end{tabularx} & \textbf{2} & \textbf{30} \\
\cmidrule[04pt]lr{2-3} &  &  \\
\begin{tabularx}{\linewidth}{Xr} The test is a one-tailed binomial test to determine probability that the strategy in the  
             column is likely to have lower accuracy in more than half of the experiments & \textbf{Test Statistics} \end{tabularx} & \textbf{p-value: < 0.00001} & \textbf{Confidence Interval:  081606 --- 1} \\


==> mev2.tex <==
 RecurrentConceptDriftStream -x 200000 -y 200000 -z 100  AgrawalGenerator -f 2 -i 2 -d AgrawalGenerator -f 3 -i 3 & \textbf{018373} & 019145 \\
 RecurrentConceptDriftStream -x 200000 -y 200000 -z 100  RandomTreeGenerator -r 1 -i 1 -d RandomTreeGenerator -r 2 -i 2 & \textbf{020024} & 020745 \\
 RecurrentConceptDriftStream -x 200000 -y 200000 -z 100  SEAGenerator -f 2 -i 2 -d SEAGenerator -f 3 -i 3 & \textbf{013948} & 01442 \\
 RecurrentConceptDriftStream -x 200000 -y 200000 -z 100  STAGGERGenerator -i 2 -f 2 -d STAGGERGenerator -i 3 -f 3 & 017949 & \textbf{017514} \\
 HyperplaneGenerator -k 10 -t 00001 -i 2 & 010626 & \textbf{010209} \\
 HyperplaneGenerator -k 10 -t 0001 -i 2 & \textbf{012861} & 014834 \\
 HyperplaneGenerator -k 10 -t 001 -i 2 & \textbf{013128} & 015154 \\
 HyperplaneGenerator -k 5 -t 00001 -i 2 & 010271 & \textbf{009573} \\
 HyperplaneGenerator -k 5 -t 0001 -i 2 & \textbf{012442} & 014618 \\
 HyperplaneGenerator -k 5 -t 001 -i 2 & \textbf{012493} & 015145 \\
 LEDGeneratorDrift -d 1 -i 2 & 026032 & \textbf{025997} \\
 LEDGeneratorDrift -d 3 -i 2 & 026032 & \textbf{025997} \\
 LEDGeneratorDrift -d 5 -i 2 & 026032 & \textbf{025997} \\
 LEDGeneratorDrift -d 7 -i 2 & 026032 & \textbf{025996} \\
 RandomRBFGeneratorDrift  00001 -k 10 -i 2 -r 2 & \textbf{007194} & 0084 \\
 RandomRBFGeneratorDrift  00001 -k 50 -i 2 -r 2 & \textbf{016055} & 018332 \\
 RandomRBFGeneratorDrift  0001 -k 10 -i 2 -r 2 & \textbf{010982} & 011502 \\
 RandomRBFGeneratorDrift  0001 -k 50 -i 2 -r 2 & 035289 & \textbf{033978} \\
 WaveformGeneratorDrift -d 1 -i 2 -n & \textbf{014411} & 014921 \\
 WaveformGeneratorDrift -d 3 -i 2 -n & \textbf{014411} & 014921 \\
 WaveformGeneratorDrift -d 5 -i 2 -n & \textbf{014411} & 014921 \\
 WaveformGeneratorDrift -d 7 -i 2 -n & \textbf{014411} & 014921 \\
 AbruptDriftGenerator -c  -o 10 -z 2 -n 2 -v 2 -r 2 -b 200000 -d Recurrent & \textbf{033746} & 033921 \\
 AbruptDriftGenerator -c  -o 10 -z 3 -n 2 -v 2 -r 2 -b 200000 -d Recurrent & \textbf{035744} & 03587 \\
 AbruptDriftGenerator -c  -o 10 -z 3 -n 3 -v 2 -r 2 -b 200000 -d Recurrent & 032838 & \textbf{032643} \\
 AbruptDriftGenerator -c  -o 10 -z 3 -n 3 -v 3 -r 2 -b 200000 -d Recurrent & \textbf{035037} & 035755 \\
 AbruptDriftGenerator -c  -o 10 -z 3 -n 3 -v 4 -r 2 -b 200000 -d Recurrent & \textbf{03698} & 038918 \\
 AbruptDriftGenerator -c  -o 10 -z 3 -n 3 -v 5 -r 2 -b 200000 -d Recurrent & \textbf{038665} & 038905 \\
 AbruptDriftGenerator -c  -o 10 -z 4 -n 2 -v 2 -r 2 -b 200000 -d Recurrent & 034205 & \textbf{032939} \\
 AbruptDriftGenerator -c  -o 10 -z 4 -n 4 -v 4 -r 2 -b 200000 -d Recurrent & \textbf{036757} & 038303 \\
 AbruptDriftGenerator -c  -o 10 -z 5 -n 2 -v 2 -r 2 -b 200000 -d Recurrent & 034167 & \textbf{032769} \\
 AbruptDriftGenerator -c  -o 10 -z 5 -n 5 -v 5 -r 2 -b 200000 -d Recurrent & \textbf{035437} & 039253 \\
\bottomrule &  &  \\
\begin{tabularx}{\linewidth}{Xr}
		A \textbf{bold} value indicates higher accuracy, and \textit{\textbf{bold italics}} indicate a tie  & \textbf{Unique Wins}
		\end{tabularx} & \textbf{21} & \textbf{11} \\
\cmidrule[04pt]lr{2-3} &  &  \\
\begin{tabularx}{\linewidth}{Xr} The test is a one-tailed binomial test to determine probability that the strategy in the  
             column is likely to have lower accuracy in more than half of the experiments & \textbf{Test Statistics} \end{tabularx} & \textbf{p-value: 097495} & \textbf{Confidence Interval:  020618 --- 1} \\


==> mev3.tex <==
 RecurrentConceptDriftStream -x 200000 -y 200000 -z 100  AgrawalGenerator -f 2 -i 2 -d AgrawalGenerator -f 3 -i 3 & \textbf{010205} & 02001 \\
 RecurrentConceptDriftStream -x 200000 -y 200000 -z 100  RandomTreeGenerator -r 1 -i 1 -d RandomTreeGenerator -r 2 -i 2 & \textbf{00642} & 019747 \\
 RecurrentConceptDriftStream -x 200000 -y 200000 -z 100  SEAGenerator -f 2 -i 2 -d SEAGenerator -f 3 -i 3 & \textbf{010639} & 014106 \\
 RecurrentConceptDriftStream -x 200000 -y 200000 -z 100  STAGGERGenerator -i 2 -f 2 -d STAGGERGenerator -i 3 -f 3 & \textbf{000141} & 019141 \\
 HyperplaneGenerator -k 10 -t 00001 -i 2 & \textbf{011024} & 01141 \\
 HyperplaneGenerator -k 10 -t 0001 -i 2 & \textbf{011736} & 016105 \\
 HyperplaneGenerator -k 10 -t 001 -i 2 & \textbf{011779} & 016447 \\
 HyperplaneGenerator -k 5 -t 00001 -i 2 & 010881 & \textbf{010639} \\
 HyperplaneGenerator -k 5 -t 0001 -i 2 & \textbf{010908} & 015599 \\
 HyperplaneGenerator -k 5 -t 001 -i 2 & \textbf{009761} & 015838 \\
 LEDGeneratorDrift -d 1 -i 2 & 028041 & \textbf{026011} \\
 LEDGeneratorDrift -d 3 -i 2 & 02804 & \textbf{026011} \\
 LEDGeneratorDrift -d 5 -i 2 & 028049 & \textbf{026011} \\
 LEDGeneratorDrift -d 7 -i 2 & 028039 & \textbf{026011} \\
 RandomRBFGeneratorDrift  00001 -k 10 -i 2 -r 2 & \textbf{006153} & 006514 \\
 RandomRBFGeneratorDrift  00001 -k 50 -i 2 -r 2 & \textbf{00825} & 015039 \\
 RandomRBFGeneratorDrift  0001 -k 10 -i 2 -r 2 & \textbf{008741} & 009594 \\
 RandomRBFGeneratorDrift  0001 -k 50 -i 2 -r 2 & \textbf{017382} & 030655 \\
 WaveformGeneratorDrift -d 1 -i 2 -n & 014862 & \textbf{014798} \\
 WaveformGeneratorDrift -d 3 -i 2 -n & 014862 & \textbf{014798} \\
 WaveformGeneratorDrift -d 5 -i 2 -n & 014862 & \textbf{014798} \\
 WaveformGeneratorDrift -d 7 -i 2 -n & 014861 & \textbf{014798} \\
 AbruptDriftGenerator -c  -o 10 -z 2 -n 2 -v 2 -r 2 -b 200000 -d Recurrent & \textbf{009068} & 032199 \\
 AbruptDriftGenerator -c  -o 10 -z 3 -n 2 -v 2 -r 2 -b 200000 -d Recurrent & \textbf{015752} & 037013 \\
 AbruptDriftGenerator -c  -o 10 -z 3 -n 3 -v 2 -r 2 -b 200000 -d Recurrent & \textbf{011655} & 034405 \\
 AbruptDriftGenerator -c  -o 10 -z 3 -n 3 -v 3 -r 2 -b 200000 -d Recurrent & \textbf{016132} & 035421 \\
 AbruptDriftGenerator -c  -o 10 -z 3 -n 3 -v 4 -r 2 -b 200000 -d Recurrent & \textbf{017869} & 039439 \\
 AbruptDriftGenerator -c  -o 10 -z 3 -n 3 -v 5 -r 2 -b 200000 -d Recurrent & \textbf{01693} & 039358 \\
 AbruptDriftGenerator -c  -o 10 -z 4 -n 2 -v 2 -r 2 -b 200000 -d Recurrent & \textbf{011094} & 031978 \\
 AbruptDriftGenerator -c  -o 10 -z 4 -n 4 -v 4 -r 2 -b 200000 -d Recurrent & \textbf{012842} & 039685 \\
 AbruptDriftGenerator -c  -o 10 -z 5 -n 2 -v 2 -r 2 -b 200000 -d Recurrent & \textbf{013362} & 033077 \\
 AbruptDriftGenerator -c  -o 10 -z 5 -n 5 -v 5 -r 2 -b 200000 -d Recurrent & \textbf{008684} & 03999 \\
\bottomrule &  &  \\
\begin{tabularx}{\linewidth}{Xr}
		A \textbf{bold} value indicates higher accuracy, and \textit{\textbf{bold italics}} indicate a tie  & \textbf{Unique Wins}
		\end{tabularx} & \textbf{23} & \textbf{9} \\
\cmidrule[04pt]lr{2-3} &  &  \\
\begin{tabularx}{\linewidth}{Xr} The test is a one-tailed binomial test to determine probability that the strategy in the  
             column is likely to have lower accuracy in more than half of the experiments & \textbf{Test Statistics} \end{tabularx} & \textbf{p-value: 09965} & \textbf{Confidence Interval:  015528 --- 1} \\


==> mev4.tex <==
 RecurrentConceptDriftStream -x 200000 -y 200000 -z 100  AgrawalGenerator -f 2 -i 2 -d AgrawalGenerator -f 3 -i 3 & \textbf{012652} & 01968 \\
 RecurrentConceptDriftStream -x 200000 -y 200000 -z 100  RandomTreeGenerator -r 1 -i 1 -d RandomTreeGenerator -r 2 -i 2 & \textbf{00846} & 021247 \\
 RecurrentConceptDriftStream -x 200000 -y 200000 -z 100  SEAGenerator -f 2 -i 2 -d SEAGenerator -f 3 -i 3 & \textbf{011262} & 014635 \\
 RecurrentConceptDriftStream -x 200000 -y 200000 -z 100  STAGGERGenerator -i 2 -f 2 -d STAGGERGenerator -i 3 -f 3 & \textbf{000299} & 017477 \\
 HyperplaneGenerator -k 10 -t 00001 -i 2 & \textbf{010371} & 010901 \\
 HyperplaneGenerator -k 10 -t 0001 -i 2 & \textbf{011387} & 015844 \\
 HyperplaneGenerator -k 10 -t 001 -i 2 & \textbf{011436} & 016092 \\
 HyperplaneGenerator -k 5 -t 00001 -i 2 & \textbf{010153} & 010194 \\
 HyperplaneGenerator -k 5 -t 0001 -i 2 & \textbf{010753} & 015448 \\
 HyperplaneGenerator -k 5 -t 001 -i 2 & \textbf{010127} & 015921 \\
 LEDGeneratorDrift -d 1 -i 2 & 02602 & \textbf{026019} \\
 LEDGeneratorDrift -d 3 -i 2 & 02602 & \textbf{026019} \\
 LEDGeneratorDrift -d 5 -i 2 & 02602 & \textbf{026019} \\
 LEDGeneratorDrift -d 7 -i 2 & 02602 & \textbf{026019} \\
 RandomRBFGeneratorDrift  00001 -k 10 -i 2 -r 2 & \textbf{007201} & 007945 \\
 RandomRBFGeneratorDrift  00001 -k 50 -i 2 -r 2 & \textbf{011136} & 018388 \\
 RandomRBFGeneratorDrift  0001 -k 10 -i 2 -r 2 & \textbf{010947} & 011286 \\
 RandomRBFGeneratorDrift  0001 -k 50 -i 2 -r 2 & \textbf{029876} & 036223 \\
 WaveformGeneratorDrift -d 1 -i 2 -n & \textbf{014413} & 014627 \\
 WaveformGeneratorDrift -d 3 -i 2 -n & \textbf{014413} & 014627 \\
 WaveformGeneratorDrift -d 5 -i 2 -n & \textbf{014413} & 014627 \\
 WaveformGeneratorDrift -d 7 -i 2 -n & \textbf{014413} & 014627 \\
 AbruptDriftGenerator -c  -o 10 -z 2 -n 2 -v 2 -r 2 -b 200000 -d Recurrent & \textbf{011331} & 03431 \\
 AbruptDriftGenerator -c  -o 10 -z 3 -n 2 -v 2 -r 2 -b 200000 -d Recurrent & \textbf{015517} & 037099 \\
 AbruptDriftGenerator -c  -o 10 -z 3 -n 3 -v 2 -r 2 -b 200000 -d Recurrent & \textbf{012188} & 03459 \\
 AbruptDriftGenerator -c  -o 10 -z 3 -n 3 -v 3 -r 2 -b 200000 -d Recurrent & \textbf{014827} & 036143 \\
 AbruptDriftGenerator -c  -o 10 -z 3 -n 3 -v 4 -r 2 -b 200000 -d Recurrent & \textbf{017691} & 039642 \\
 AbruptDriftGenerator -c  -o 10 -z 3 -n 3 -v 5 -r 2 -b 200000 -d Recurrent & \textbf{015904} & 039614 \\
 AbruptDriftGenerator -c  -o 10 -z 4 -n 2 -v 2 -r 2 -b 200000 -d Recurrent & \textbf{01336} & 034057 \\
 AbruptDriftGenerator -c  -o 10 -z 4 -n 4 -v 4 -r 2 -b 200000 -d Recurrent & \textbf{015267} & 040099 \\
 AbruptDriftGenerator -c  -o 10 -z 5 -n 2 -v 2 -r 2 -b 200000 -d Recurrent & \textbf{011422} & 033857 \\
 AbruptDriftGenerator -c  -o 10 -z 5 -n 5 -v 5 -r 2 -b 200000 -d Recurrent & \textbf{015781} & 040625 \\
\bottomrule &  &  \\
\begin{tabularx}{\linewidth}{Xr}
		A \textbf{bold} value indicates higher accuracy, and \textit{\textbf{bold italics}} indicate a tie  & \textbf{Unique Wins}
		\end{tabularx} & \textbf{28} & \textbf{4} \\
\cmidrule[04pt]lr{2-3} &  &  \\
\begin{tabularx}{\linewidth}{Xr} The test is a one-tailed binomial test to determine probability that the strategy in the  
             column is likely to have lower accuracy in more than half of the experiments & \textbf{Test Statistics} \end{tabularx} & \textbf{p-value: 1} & \textbf{Confidence Interval:  004385 --- 1} \\


==> mev5.tex <==
 RecurrentConceptDriftStream -x 200000 -y 200000 -z 100  AgrawalGenerator -f 2 -i 2 -d AgrawalGenerator -f 3 -i 3 & 017084 & \textbf{015346} \\
 RecurrentConceptDriftStream -x 200000 -y 200000 -z 100  RandomTreeGenerator -r 1 -i 1 -d RandomTreeGenerator -r 2 -i 2 & 013912 & \textbf{01323} \\
 RecurrentConceptDriftStream -x 200000 -y 200000 -z 100  SEAGenerator -f 2 -i 2 -d SEAGenerator -f 3 -i 3 & 012015 & \textbf{011841} \\
 RecurrentConceptDriftStream -x 200000 -y 200000 -z 100  STAGGERGenerator -i 2 -f 2 -d STAGGERGenerator -i 3 -f 3 & 009834 & \textbf{006311} \\
 HyperplaneGenerator -k 10 -t 00001 -i 2 & \textbf{011168} & 011396 \\
 HyperplaneGenerator -k 10 -t 0001 -i 2 & 012744 & \textbf{012698} \\
 HyperplaneGenerator -k 10 -t 001 -i 2 & 012851 & \textbf{01275} \\
 HyperplaneGenerator -k 5 -t 00001 -i 2 & \textbf{011004} & 011241 \\
 HyperplaneGenerator -k 5 -t 0001 -i 2 & 012168 & \textbf{011813} \\
 HyperplaneGenerator -k 5 -t 001 -i 2 & 011479 & \textbf{01105} \\
 LEDGeneratorDrift -d 1 -i 2 & \textbf{026009} & 02601 \\
 LEDGeneratorDrift -d 3 -i 2 & \textbf{026009} & 026011 \\
 LEDGeneratorDrift -d 5 -i 2 & \textbf{026009} & 026011 \\
 LEDGeneratorDrift -d 7 -i 2 & \textbf{026009} & 026015 \\
 RandomRBFGeneratorDrift  00001 -k 10 -i 2 -r 2 & 006694 & \textbf{006479} \\
 RandomRBFGeneratorDrift  00001 -k 50 -i 2 -r 2 & 013939 & \textbf{013468} \\
 RandomRBFGeneratorDrift  0001 -k 10 -i 2 -r 2 & 010173 & \textbf{009913} \\
 RandomRBFGeneratorDrift  0001 -k 50 -i 2 -r 2 & 03171 & \textbf{031099} \\
 WaveformGeneratorDrift -d 1 -i 2 -n & 016145 & \textbf{016057} \\
 WaveformGeneratorDrift -d 3 -i 2 -n & 016145 & \textbf{01605} \\
 WaveformGeneratorDrift -d 5 -i 2 -n & 016145 & \textbf{016053} \\
 WaveformGeneratorDrift -d 7 -i 2 -n & 016141 & \textbf{016047} \\
 AbruptDriftGenerator -c  -o 10 -z 2 -n 2 -v 2 -r 2 -b 200000 -d Recurrent & \textbf{012248} & 012743 \\
 AbruptDriftGenerator -c  -o 10 -z 3 -n 2 -v 2 -r 2 -b 200000 -d Recurrent & 01498 & \textbf{012291} \\
 AbruptDriftGenerator -c  -o 10 -z 3 -n 3 -v 2 -r 2 -b 200000 -d Recurrent & 012366 & \textbf{005914} \\
 AbruptDriftGenerator -c  -o 10 -z 3 -n 3 -v 3 -r 2 -b 200000 -d Recurrent & 017282 & \textbf{010713} \\
 AbruptDriftGenerator -c  -o 10 -z 3 -n 3 -v 4 -r 2 -b 200000 -d Recurrent & 017083 & \textbf{008965} \\
 AbruptDriftGenerator -c  -o 10 -z 3 -n 3 -v 5 -r 2 -b 200000 -d Recurrent & 016706 & \textbf{00949} \\
 AbruptDriftGenerator -c  -o 10 -z 4 -n 2 -v 2 -r 2 -b 200000 -d Recurrent & 015191 & \textbf{014134} \\
 AbruptDriftGenerator -c  -o 10 -z 4 -n 4 -v 4 -r 2 -b 200000 -d Recurrent & 011737 & \textbf{003993} \\
 AbruptDriftGenerator -c  -o 10 -z 5 -n 2 -v 2 -r 2 -b 200000 -d Recurrent & \textbf{012386} & 013373 \\
 AbruptDriftGenerator -c  -o 10 -z 5 -n 5 -v 5 -r 2 -b 200000 -d Recurrent & 029368 & \textbf{007874} \\
\bottomrule &  &  \\
\begin{tabularx}{\linewidth}{Xr}
		A \textbf{bold} value indicates higher accuracy, and \textit{\textbf{bold italics}} indicate a tie  & \textbf{Unique Wins}
		\end{tabularx} & \textbf{8} & \textbf{24} \\
\cmidrule[04pt]lr{2-3} &  &  \\
\begin{tabularx}{\linewidth}{Xr} The test is a one-tailed binomial test to determine probability that the strategy in the  
             column is likely to have lower accuracy in more than half of the experiments & \textbf{Test Statistics} \end{tabularx} & \textbf{p-value: 00035} & \textbf{Confidence Interval:  059394 --- 1} \\


==> mev6.tex <==
 RecurrentConceptDriftStream -x 200000 -y 200000 -z 100  AgrawalGenerator -f 2 -i 2 -d AgrawalGenerator -f 3 -i 3 & 017084 & \textbf{015346} \\
 RecurrentConceptDriftStream -x 200000 -y 200000 -z 100  RandomTreeGenerator -r 1 -i 1 -d RandomTreeGenerator -r 2 -i 2 & 013912 & \textbf{01323} \\
 RecurrentConceptDriftStream -x 200000 -y 200000 -z 100  SEAGenerator -f 2 -i 2 -d SEAGenerator -f 3 -i 3 & 012015 & \textbf{011842} \\
 RecurrentConceptDriftStream -x 200000 -y 200000 -z 100  STAGGERGenerator -i 2 -f 2 -d STAGGERGenerator -i 3 -f 3 & 009834 & \textbf{006311} \\
 HyperplaneGenerator -k 10 -t 00001 -i 2 & \textbf{011168} & 011396 \\
 HyperplaneGenerator -k 10 -t 0001 -i 2 & 012744 & \textbf{012698} \\
 HyperplaneGenerator -k 10 -t 001 -i 2 & 012851 & \textbf{01275} \\
 HyperplaneGenerator -k 5 -t 00001 -i 2 & \textbf{011004} & 011241 \\
 HyperplaneGenerator -k 5 -t 0001 -i 2 & 012168 & \textbf{011813} \\
 HyperplaneGenerator -k 5 -t 001 -i 2 & 011479 & \textbf{01105} \\
 LEDGeneratorDrift -d 1 -i 2 & \textbf{026011} & 026013 \\
 LEDGeneratorDrift -d 3 -i 2 & \textbf{026011} & 026014 \\
 LEDGeneratorDrift -d 5 -i 2 & \textbf{026011} & 026014 \\
 LEDGeneratorDrift -d 7 -i 2 & \textbf{026011} & 026017 \\
 RandomRBFGeneratorDrift  00001 -k 10 -i 2 -r 2 & 006694 & \textbf{006479} \\
 RandomRBFGeneratorDrift  00001 -k 50 -i 2 -r 2 & 013939 & \textbf{013468} \\
 RandomRBFGeneratorDrift  0001 -k 10 -i 2 -r 2 & 010173 & \textbf{009913} \\
 RandomRBFGeneratorDrift  0001 -k 50 -i 2 -r 2 & 03171 & \textbf{031098} \\
 WaveformGeneratorDrift -d 1 -i 2 -n & 016145 & \textbf{016057} \\
 WaveformGeneratorDrift -d 3 -i 2 -n & 016145 & \textbf{01605} \\
 WaveformGeneratorDrift -d 5 -i 2 -n & 016145 & \textbf{016053} \\
 WaveformGeneratorDrift -d 7 -i 2 -n & 016142 & \textbf{016047} \\
 AbruptDriftGenerator -c  -o 10 -z 2 -n 2 -v 2 -r 2 -b 200000 -d Recurrent & \textbf{012251} & 012888 \\
 AbruptDriftGenerator -c  -o 10 -z 3 -n 2 -v 2 -r 2 -b 200000 -d Recurrent & 015083 & \textbf{012394} \\
 AbruptDriftGenerator -c  -o 10 -z 3 -n 3 -v 2 -r 2 -b 200000 -d Recurrent & 012366 & \textbf{005914} \\
 AbruptDriftGenerator -c  -o 10 -z 3 -n 3 -v 3 -r 2 -b 200000 -d Recurrent & 017282 & \textbf{010713} \\
 AbruptDriftGenerator -c  -o 10 -z 3 -n 3 -v 4 -r 2 -b 200000 -d Recurrent & 017084 & \textbf{008981} \\
 AbruptDriftGenerator -c  -o 10 -z 3 -n 3 -v 5 -r 2 -b 200000 -d Recurrent & 01672 & \textbf{009548} \\
 AbruptDriftGenerator -c  -o 10 -z 4 -n 2 -v 2 -r 2 -b 200000 -d Recurrent & 015191 & \textbf{014134} \\
 AbruptDriftGenerator -c  -o 10 -z 4 -n 4 -v 4 -r 2 -b 200000 -d Recurrent & 011911 & \textbf{004105} \\
 AbruptDriftGenerator -c  -o 10 -z 5 -n 2 -v 2 -r 2 -b 200000 -d Recurrent & \textbf{01249} & 013476 \\
 AbruptDriftGenerator -c  -o 10 -z 5 -n 5 -v 5 -r 2 -b 200000 -d Recurrent & 032364 & \textbf{008112} \\
\bottomrule &  &  \\
\begin{tabularx}{\linewidth}{Xr}
		A \textbf{bold} value indicates higher accuracy, and \textit{\textbf{bold italics}} indicate a tie  & \textbf{Unique Wins}
		\end{tabularx} & \textbf{8} & \textbf{24} \\
\cmidrule[04pt]lr{2-3} &  &  \\
\begin{tabularx}{\linewidth}{Xr} The test is a one-tailed binomial test to determine probability that the strategy in the  
             column is likely to have lower accuracy in more than half of the experiments & \textbf{Test Statistics} \end{tabularx} & \textbf{p-value: 00035} & \textbf{Confidence Interval:  059394 --- 1} \\


==> mev7.tex <==
 RecurrentConceptDriftStream -x 200000 -y 200000 -z 100  AgrawalGenerator -f 2 -i 2 -d AgrawalGenerator -f 3 -i 3 & 015742 & \textbf{011929} \\
 RecurrentConceptDriftStream -x 200000 -y 200000 -z 100  RandomTreeGenerator -r 1 -i 1 -d RandomTreeGenerator -r 2 -i 2 & 013294 & \textbf{009511} \\
 RecurrentConceptDriftStream -x 200000 -y 200000 -z 100  SEAGenerator -f 2 -i 2 -d SEAGenerator -f 3 -i 3 & 012719 & \textbf{011452} \\
 RecurrentConceptDriftStream -x 200000 -y 200000 -z 100  STAGGERGenerator -i 2 -f 2 -d STAGGERGenerator -i 3 -f 3 & 008442 & \textbf{000172} \\
 HyperplaneGenerator -k 10 -t 00001 -i 2 & 011215 & \textbf{010114} \\
 HyperplaneGenerator -k 10 -t 0001 -i 2 & 012523 & \textbf{010998} \\
 HyperplaneGenerator -k 10 -t 001 -i 2 & 012565 & \textbf{011091} \\
 HyperplaneGenerator -k 5 -t 00001 -i 2 & 011043 & \textbf{009972} \\
 HyperplaneGenerator -k 5 -t 0001 -i 2 & 011864 & \textbf{010515} \\
 HyperplaneGenerator -k 5 -t 001 -i 2 & 011393 & \textbf{010014} \\
 LEDGeneratorDrift -d 1 -i 2 & 026109 & \textbf{025996} \\
 LEDGeneratorDrift -d 3 -i 2 & 026109 & \textbf{025996} \\
 LEDGeneratorDrift -d 5 -i 2 & 026109 & \textbf{025996} \\
 LEDGeneratorDrift -d 7 -i 2 & 026109 & \textbf{025996} \\
 RandomRBFGeneratorDrift  00001 -k 10 -i 2 -r 2 & \textbf{006664} & 007738 \\
 RandomRBFGeneratorDrift  00001 -k 50 -i 2 -r 2 & 013559 & \textbf{013282} \\
 RandomRBFGeneratorDrift  0001 -k 10 -i 2 -r 2 & \textbf{010126} & 011143 \\
 RandomRBFGeneratorDrift  0001 -k 50 -i 2 -r 2 & 031195 & \textbf{030834} \\
 WaveformGeneratorDrift -d 1 -i 2 -n & 015871 & \textbf{014594} \\
 WaveformGeneratorDrift -d 3 -i 2 -n & 015872 & \textbf{014594} \\
 WaveformGeneratorDrift -d 5 -i 2 -n & 015872 & \textbf{014594} \\
 WaveformGeneratorDrift -d 7 -i 2 -n & 015872 & \textbf{014594} \\
 AbruptDriftGenerator -c  -o 10 -z 2 -n 2 -v 2 -r 2 -b 200000 -d Recurrent & 022166 & \textbf{012285} \\
 AbruptDriftGenerator -c  -o 10 -z 3 -n 2 -v 2 -r 2 -b 200000 -d Recurrent & 017571 & \textbf{016658} \\
 AbruptDriftGenerator -c  -o 10 -z 3 -n 3 -v 2 -r 2 -b 200000 -d Recurrent & \textbf{009681} & 011804 \\
 AbruptDriftGenerator -c  -o 10 -z 3 -n 3 -v 3 -r 2 -b 200000 -d Recurrent & \textbf{011988} & 014935 \\
 AbruptDriftGenerator -c  -o 10 -z 3 -n 3 -v 4 -r 2 -b 200000 -d Recurrent & \textbf{010993} & 01531 \\
 AbruptDriftGenerator -c  -o 10 -z 3 -n 3 -v 5 -r 2 -b 200000 -d Recurrent & \textbf{012118} & 018661 \\
 AbruptDriftGenerator -c  -o 10 -z 4 -n 2 -v 2 -r 2 -b 200000 -d Recurrent & 018369 & \textbf{012408} \\
 AbruptDriftGenerator -c  -o 10 -z 4 -n 4 -v 4 -r 2 -b 200000 -d Recurrent & \textbf{005954} & 017194 \\
 AbruptDriftGenerator -c  -o 10 -z 5 -n 2 -v 2 -r 2 -b 200000 -d Recurrent & 018467 & \textbf{011097} \\
 AbruptDriftGenerator -c  -o 10 -z 5 -n 5 -v 5 -r 2 -b 200000 -d Recurrent & \textbf{011939} & 029009 \\
\bottomrule &  &  \\
\begin{tabularx}{\linewidth}{Xr}
		A \textbf{bold} value indicates higher accuracy, and \textit{\textbf{bold italics}} indicate a tie  & \textbf{Unique Wins}
		\end{tabularx} & \textbf{8} & \textbf{24} \\
\cmidrule[04pt]lr{2-3} &  &  \\
\begin{tabularx}{\linewidth}{Xr} The test is a one-tailed binomial test to determine probability that the strategy in the  
             column is likely to have lower accuracy in more than half of the experiments & \textbf{Test Statistics} \end{tabularx} & \textbf{p-value: 00035} & \textbf{Confidence Interval:  059394 --- 1} \\


==> mev8.tex <==
 RecurrentConceptDriftStream -x 200000 -y 200000 -z 100  AgrawalGenerator -f 2 -i 2 -d AgrawalGenerator -f 3 -i 3 & \textbf{01748} & 01812 \\
 RecurrentConceptDriftStream -x 200000 -y 200000 -z 100  RandomTreeGenerator -r 1 -i 1 -d RandomTreeGenerator -r 2 -i 2 & \textbf{012445} & 014317 \\
 RecurrentConceptDriftStream -x 200000 -y 200000 -z 100  SEAGenerator -f 2 -i 2 -d SEAGenerator -f 3 -i 3 & 01449 & \textbf{013049} \\
 RecurrentConceptDriftStream -x 200000 -y 200000 -z 100  STAGGERGenerator -i 2 -f 2 -d STAGGERGenerator -i 3 -f 3 & \textbf{001347} & 010382 \\
 HyperplaneGenerator -k 10 -t 00001 -i 2 & 015898 & \textbf{010869} \\
 HyperplaneGenerator -k 10 -t 0001 -i 2 & 016057 & \textbf{013259} \\
 HyperplaneGenerator -k 10 -t 001 -i 2 & 016392 & \textbf{013299} \\
 HyperplaneGenerator -k 5 -t 00001 -i 2 & 015808 & \textbf{010511} \\
 HyperplaneGenerator -k 5 -t 0001 -i 2 & 014838 & \textbf{012736} \\
 HyperplaneGenerator -k 5 -t 001 -i 2 & 013675 & \textbf{012153} \\
 LEDGeneratorDrift -d 1 -i 2 & 026164 & \textbf{026119} \\
 LEDGeneratorDrift -d 3 -i 2 & \textbf{026109} & 026119 \\
 LEDGeneratorDrift -d 5 -i 2 & \textbf{026107} & 026119 \\
 LEDGeneratorDrift -d 7 -i 2 & 026169 & \textbf{026119} \\
 RandomRBFGeneratorDrift  00001 -k 10 -i 2 -r 2 & 007398 & \textbf{006847} \\
 RandomRBFGeneratorDrift  00001 -k 50 -i 2 -r 2 & \textbf{011857} & 014149 \\
 RandomRBFGeneratorDrift  0001 -k 10 -i 2 -r 2 & 010793 & \textbf{010352} \\
 RandomRBFGeneratorDrift  0001 -k 50 -i 2 -r 2 & \textbf{022421} & 031758 \\
 WaveformGeneratorDrift -d 1 -i 2 -n & 018216 & \textbf{015797} \\
 WaveformGeneratorDrift -d 3 -i 2 -n & 018155 & \textbf{015797} \\
 WaveformGeneratorDrift -d 5 -i 2 -n & 018087 & \textbf{015797} \\
 WaveformGeneratorDrift -d 7 -i 2 -n & 018123 & \textbf{015795} \\
 AbruptDriftGenerator -c  -o 10 -z 2 -n 2 -v 2 -r 2 -b 200000 -d Recurrent & \textbf{009672} & 024091 \\
 AbruptDriftGenerator -c  -o 10 -z 3 -n 2 -v 2 -r 2 -b 200000 -d Recurrent & \textbf{003094} & 021457 \\
 AbruptDriftGenerator -c  -o 10 -z 3 -n 3 -v 2 -r 2 -b 200000 -d Recurrent & \textbf{000031} & 02061 \\
 AbruptDriftGenerator -c  -o 10 -z 3 -n 3 -v 3 -r 2 -b 200000 -d Recurrent & \textbf{000042} & 021236 \\
 AbruptDriftGenerator -c  -o 10 -z 3 -n 3 -v 4 -r 2 -b 200000 -d Recurrent & \textbf{000093} & 021905 \\
 AbruptDriftGenerator -c  -o 10 -z 3 -n 3 -v 5 -r 2 -b 200000 -d Recurrent & \textbf{00023} & 021731 \\
 AbruptDriftGenerator -c  -o 10 -z 4 -n 2 -v 2 -r 2 -b 200000 -d Recurrent & \textbf{002032} & 02311 \\
 AbruptDriftGenerator -c  -o 10 -z 4 -n 4 -v 4 -r 2 -b 200000 -d Recurrent & \textbf{001399} & 02074 \\
 AbruptDriftGenerator -c  -o 10 -z 5 -n 2 -v 2 -r 2 -b 200000 -d Recurrent & \textbf{00188} & 02181 \\
 AbruptDriftGenerator -c  -o 10 -z 5 -n 5 -v 5 -r 2 -b 200000 -d Recurrent & \textbf{017661} & 03756 \\
\bottomrule &  &  \\
\begin{tabularx}{\linewidth}{Xr}
		A \textbf{bold} value indicates higher accuracy, and \textit{\textbf{bold italics}} indicate a tie  & \textbf{Unique Wins}
		\end{tabularx} & \textbf{17} & \textbf{15} \\
\cmidrule[04pt]lr{2-3} &  &  \\
\begin{tabularx}{\linewidth}{Xr} The test is a one-tailed binomial test to determine probability that the strategy in the  
             column is likely to have lower accuracy in more than half of the experiments & \textbf{Test Statistics} \end{tabularx} & \textbf{p-value: 070169} & \textbf{Confidence Interval:  031544 --- 1} \\


==> mev9.tex <==
 RecurrentConceptDriftStream -x 200000 -y 200000 -z 100  AgrawalGenerator -f 2 -i 2 -d AgrawalGenerator -f 3 -i 3 & 017937 & \textbf{011408} \\
 RecurrentConceptDriftStream -x 200000 -y 200000 -z 100  RandomTreeGenerator -r 1 -i 1 -d RandomTreeGenerator -r 2 -i 2 & 019807 & \textbf{006448} \\
 RecurrentConceptDriftStream -x 200000 -y 200000 -z 100  SEAGenerator -f 2 -i 2 -d SEAGenerator -f 3 -i 3 & 013578 & \textbf{010672} \\
 RecurrentConceptDriftStream -x 200000 -y 200000 -z 100  STAGGERGenerator -i 2 -f 2 -d STAGGERGenerator -i 3 -f 3 & 018746 & \textbf{000137} \\
 HyperplaneGenerator -k 10 -t 00001 -i 2 & \textbf{0098} & 010714 \\
 HyperplaneGenerator -k 10 -t 0001 -i 2 & 012153 & \textbf{011543} \\
 HyperplaneGenerator -k 10 -t 001 -i 2 & 012284 & \textbf{011623} \\
 HyperplaneGenerator -k 5 -t 00001 -i 2 & \textbf{009475} & 010488 \\
 HyperplaneGenerator -k 5 -t 0001 -i 2 & 01171 & \textbf{010807} \\
 HyperplaneGenerator -k 5 -t 001 -i 2 & 012062 & \textbf{009741} \\
 LEDGeneratorDrift -d 1 -i 2 & 026066 & \textbf{026033} \\
 LEDGeneratorDrift -d 3 -i 2 & 026066 & \textbf{026033} \\
 LEDGeneratorDrift -d 5 -i 2 & 026066 & \textbf{026033} \\
 LEDGeneratorDrift -d 7 -i 2 & 026066 & \textbf{026033} \\
 RandomRBFGeneratorDrift  00001 -k 10 -i 2 -r 2 & 007305 & \textbf{00605} \\
 RandomRBFGeneratorDrift  00001 -k 50 -i 2 -r 2 & 015977 & \textbf{008728} \\
 RandomRBFGeneratorDrift  0001 -k 10 -i 2 -r 2 & 010907 & \textbf{008917} \\
 RandomRBFGeneratorDrift  0001 -k 50 -i 2 -r 2 & 033032 & \textbf{018823} \\
 WaveformGeneratorDrift -d 1 -i 2 -n & \textbf{014513} & 014674 \\
 WaveformGeneratorDrift -d 3 -i 2 -n & \textbf{014513} & 014674 \\
 WaveformGeneratorDrift -d 5 -i 2 -n & \textbf{014513} & 014674 \\
 WaveformGeneratorDrift -d 7 -i 2 -n & \textbf{014513} & 014674 \\
 AbruptDriftGenerator -c  -o 10 -z 2 -n 2 -v 2 -r 2 -b 200000 -d Recurrent & 033905 & \textbf{008568} \\
 AbruptDriftGenerator -c  -o 10 -z 3 -n 2 -v 2 -r 2 -b 200000 -d Recurrent & 036061 & \textbf{015231} \\
 AbruptDriftGenerator -c  -o 10 -z 3 -n 3 -v 2 -r 2 -b 200000 -d Recurrent & 030822 & \textbf{011588} \\
 AbruptDriftGenerator -c  -o 10 -z 3 -n 3 -v 3 -r 2 -b 200000 -d Recurrent & 034818 & \textbf{015151} \\
 AbruptDriftGenerator -c  -o 10 -z 3 -n 3 -v 4 -r 2 -b 200000 -d Recurrent & 035711 & \textbf{021071} \\
 AbruptDriftGenerator -c  -o 10 -z 3 -n 3 -v 5 -r 2 -b 200000 -d Recurrent & 037848 & \textbf{020627} \\
 AbruptDriftGenerator -c  -o 10 -z 4 -n 2 -v 2 -r 2 -b 200000 -d Recurrent & 032422 & \textbf{010922} \\
 AbruptDriftGenerator -c  -o 10 -z 4 -n 4 -v 4 -r 2 -b 200000 -d Recurrent & 036083 & \textbf{017353} \\
 AbruptDriftGenerator -c  -o 10 -z 5 -n 2 -v 2 -r 2 -b 200000 -d Recurrent & 032929 & \textbf{011904} \\
 AbruptDriftGenerator -c  -o 10 -z 5 -n 5 -v 5 -r 2 -b 200000 -d Recurrent & 034937 & \textbf{013153} \\
\bottomrule &  &  \\
\begin{tabularx}{\linewidth}{Xr}
		A \textbf{bold} value indicates higher accuracy, and \textit{\textbf{bold italics}} indicate a tie  & \textbf{Unique Wins}
		\end{tabularx} & \textbf{6} & \textbf{26} \\
\cmidrule[04pt]lr{2-3} &  &  \\
\begin{tabularx}{\linewidth}{Xr} The test is a one-tailed binomial test to determine probability that the strategy in the  
             column is likely to have lower accuracy in more than half of the experiments & \textbf{Test Statistics} \end{tabularx} & \textbf{p-value: 000027} & \textbf{Confidence Interval:  066313 --- 1} \\


==> mevreal11.tex <==
-s (ArffFileStream -f /home/cman39/p2016030006/cman39/datasets/airlines/airlines.arff -c -1) & \textbf{0.34316} & 0.34607 \\
-s (ArffFileStream -f /home/cman39/p2016030006/cman39/datasets/aws/aws_discrete.arff -c -1) & 0.13038 & \textbf{0.12272} \\
-s (ArffFileStream -f /home/cman39/p2016030006/cman39/datasets/chess/chess.arff -c -1) & 0.01576 & \textbf{0.01355} \\
-s (ArffFileStream -f /home/cman39/p2016030006/cman39/datasets/covtype/covtype.arff) & 0.09768 & \textbf{0.06784} \\
-s (ArffFileStream -f /home/cman39/p2016030006/cman39/datasets/cpe/cpe.arff -c -1) & 0.17382 & \textbf{0.13015} \\
-s (ArffFileStream -f /home/cman39/p2016030006/cman39/datasets/fonts/fonts.arff -c 1) & 0.00114 & \textbf{0.00067} \\
-s (ArffFileStream -f /home/cman39/p2016030006/cman39/datasets/harpagwag/harpagwag.arff -c -1) & 0.00088 & \textbf{0.00063} \\
-s (ArffFileStream -f /home/cman39/p2016030006/cman39/datasets/kdd/kdd.arff -c -1) & \textbf{0.00034} & 0.00037 \\
-s (ArffFileStream -f /home/cman39/p2016030006/cman39/datasets/localization/localization.arff -c -1) & 0.03834 & \textbf{0.03781} \\
-s (ArffFileStream -f /home/cman39/p2016030006/cman39/datasets/miniboone/miniboone.arff -c -1) & \textbf{4e-05} & 5e-05 \\
-s (ArffFileStream -f /home/cman39/p2016030006/cman39/datasets/nbaiot/nbaiot.arff -c -1) & 9e-05 & \textbf{8e-05} \\
-s (ArffFileStream -f /home/cman39/p2016030006/cman39/datasets/nswelec/elec.arff -c -1) & 0.11276 & \textbf{0.10457} \\
-s (ArffFileStream -f /home/cman39/p2016030006/cman39/datasets/pamap2/pamap2_9subjects_.arff -c 2) & 0.003 & \textbf{0.00138} \\
-s (ArffFileStream -f /home/cman39/p2016030006/cman39/datasets/poker/poker.arff -c -1) & 0.222 & \textbf{0.1684} \\
-s (ArffFileStream -f /home/cman39/p2016030006/cman39/datasets/posturespucrio/pucrio.arff -c -1) & \textbf{0.00101} & 0.00103 \\
-s (ArffFileStream -f /home/cman39/p2016030006/cman39/datasets/sensor/sensor.arff -c -1) & 3e-04 & \textbf{0.00025} \\
-s (ArffFileStream -f /home/cman39/p2016030006/cman39/datasets/sensortemp2019/gassensor2019discretized.arff -c 2) & \textbf{0.01412} & 0.0142 \\
-s (ArffFileStream -f /home/cman39/p2016030006/cman39/datasets/skin/skin.arff -c -1) & \textit{\textbf{0.00014}} & \textit{\textbf{0.00014}} \\
-s (ArffFileStream -f /home/cman39/p2016030006/cman39/datasets/tnelec/eb.arff -c 3) & \textit{\textbf{0.00267}} & \textit{\textbf{0.00267}} \\
-s (ArffFileStream -f /home/cman39/p2016030006/cman39/datasets/wisdm/wisdm.arff -c -1) & 0.10197 & \textbf{0.06728} \\
\bottomrule &  &  \\
\begin{tabularx}{\linewidth}{Xr}
		A \textbf{bold} value indicates higher accuracy, and \textit{\textbf{bold italics}} indicate a tie.  & \textbf{Unique Wins}
		\end{tabularx} & \textbf{5} & \textbf{13} \\
\cmidrule[0.4pt](lr){2-3} &  &  \\
\begin{tabularx}{\linewidth}{Xr} The test is a one-tailed binomial test to determine the probability that the strategy in the rightmost column would achieve so many wins if wins and losses were equiprobable. & \textbf{Test Statistics} \end{tabularx} & \textbf{p-value: 0.04813} & \textbf{Confidence Interval:  0.50217 --- 1} \\


==> mevreal500.tex <==
airlines & 0.34871 & 8523 & \textbf{0.33825} & 17552 \\
aws---price-discretized & 0.14671 & 5055 & \textbf{0.14015} & 6140 \\
chess & 0.61045 & 6 & \textbf{0.287} & 71 \\
covertype & 0.1376 & 167 & \textbf{0.1078} & 208 \\
covpokelec & 0.13863 & 314 & \textbf{0.13031} & 273 \\
fonts & 0.01747 & 208 & \textbf{0.00244} & 215 \\
hhar & 0.02226 & 2385 & \textbf{0.00113} & 1250 \\
kdd & 9e-04 & 133 & \textbf{0.00089} & 177 \\
localization & 0.0941 & 159 & \textbf{0.06445} & 72 \\
miniboone & \textit{\textbf{6e-05}} & 4 & \textit{\textbf{6e-05}} & 4 \\
nbaiot & 0.00499 & 42 & \textbf{0.00117} & 28 \\
nswelec & 0.17263 & 38 & \textbf{0.17124} & 52 \\
pamap2 & 0.02873 & 165 & \textbf{0.01236} & 111 \\
poker & 0.15696 & 127 & \textbf{0.14787} & 87 \\
pucrio & 0.0191 & 22 & \textbf{0.00096} & 9 \\
sensor---home-activity & 0.00115 & 238 & \textbf{5e-04} & 19 \\
sensor---CO-discretized & \textbf{0.0125} & 593 & 0.03806 & 480 \\
skin & \textbf{0.00052} & 4 & 0.00053 & 4 \\
tnelec & \textbf{0.00254} & 2 & 0.0055 & 8 \\
wisdm & 0.10437 & 2502 & \textbf{0.07743} & 2149 \\
\midrule
\textbf{Unique Wins} & \multicolumn{2}{l?}{\textbf{3}} & \multicolumn{2}{l}{\textbf{16}} \\
\midrule\multicolumn{5}{l}{A \textbf{bold} error value indicates higher accuracy, and \textit{\textbf{bold italics}} indicate a tie.}\\
\multicolumn{5}{l}{\textbf{One-tailed binomial test statistics}:  \textbf{p-value: 0.00221};   \textbf{Confidence Interval:  0.64057 --- 1} }\\


==> mevreal501.tex <==
airlines & \textbf{0.32888} & 3470 & 0.33137 & 5057 \\
aws---price-discretized & 0.14678 & 4997 & \textbf{0.14028} & 6059 \\
chess & 0.04059 & 4 & \textbf{0.01645} & 6 \\
covertype & 0.15279 & 2 & \textbf{0.08658} & 5 \\
covpokelec & 0.21615 & 2 & \textbf{0.17651} & 2 \\
fonts & 0.0015 & 193 & \textbf{0.00078} & 193 \\
hhar & 0.01266 & 5 & \textbf{0.00102} & 7 \\
kdd & 0.00072 & 49 & \textbf{0.00069} & 47 \\
localization & 0.07885 & 11 & \textbf{0.05004} & 9 \\
miniboone & \textit{\textbf{6e-05}} & 3 & \textit{\textbf{6e-05}} & 3 \\
nbaiot & 0.00137 & 3 & \textbf{0.00027} & 4 \\
nswelec & 0.15963 & 6 & \textbf{0.12785} & 12 \\
pamap2 & 0.01703 & 2 & \textbf{0.00422} & 2 \\
poker & 0.25846 & 1 & \textbf{0.23523} & 6 \\
pucrio & 0.00106 & 2 & \textbf{0.00079} & 5 \\
sensor---home-activity & \textit{\textbf{0.00034}} & 2 & \textit{\textbf{0.00034}} & 2 \\
sensor---CO-discretized & 0.03553 & 6 & \textbf{0.02663} & 6 \\
skin & \textbf{0.00047} & 4 & 0.00048 & 3 \\
tnelec & \textbf{0.00265} & 6 & 0.00383 & 14 \\
wisdm & 0.11306 & 5 & \textbf{0.07264} & 21 \\
\midrule
\textbf{Unique Wins} & \multicolumn{2}{l?}{\textbf{3}} & \multicolumn{2}{l}{\textbf{15}} \\
\midrule\multicolumn{5}{l}{A \textbf{bold} error value indicates higher accuracy, and \textit{\textbf{bold italics}} indicate a tie.}\\
\multicolumn{5}{l}{\textbf{One-tailed binomial test statistics}:  \textbf{p-value: 0.00377};   \textbf{Confidence Interval:  0.62332 --- 1} }\\


==> mevreal5010.tex <==
airlines & 0.34955 & 8420 & \textbf{0.34782} & 14361 \\
aws---price-discretized & 0.14728 & 5041 & \textbf{0.14143} & 6144 \\
chess & 0.65807 & 5 & \textbf{0.31152} & 76 \\
covertype & 0.18905 & 217 & \textbf{0.15431} & 389 \\
covpokelec & \textbf{0.18665} & 368 & 0.19391 & 505 \\
fonts & 0.01781 & 207 & \textbf{0.003} & 211 \\
hhar & 0.03749 & 2590 & \textbf{0.00357} & 2947 \\
kdd & \textbf{0.00093} & 141 & 0.00094 & 181 \\
localization & 0.13299 & 177 & \textbf{0.09754} & 115 \\
miniboone & \textbf{0.00011} & 4 & 0.00013 & 4 \\
nbaiot & 0.00368 & 36 & \textbf{0.00076} & 29 \\
nswelec & 0.19861 & 40 & \textbf{0.19283} & 71 \\
pamap2 & 0.0972 & 234 & \textbf{0.06136} & 88 \\
poker & \textbf{0.20509} & 142 & 0.218 & 150 \\
pucrio & 0.01457 & 26 & \textbf{0.00147} & 12 \\
sensor---home-activity & 0.00906 & 238 & \textbf{0.00135} & 39 \\
sensor---CO-discretized & \textbf{0.02633} & 605 & 0.06655 & 794 \\
skin & \textbf{0.00052} & 4 & 0.00055 & 4 \\
tnelec & \textbf{0.00235} & 2 & 0.00496 & 7 \\
wisdm & 0.18796 & 2752 & \textbf{0.14576} & 2598 \\
\midrule
\textbf{Unique Wins} & \multicolumn{2}{l?}{\textbf{7}} & \multicolumn{2}{l}{\textbf{13}} \\
\midrule\multicolumn{5}{l}{A \textbf{bold} error value indicates higher accuracy, and \textit{\textbf{bold italics}} indicate a tie.}\\
\multicolumn{5}{l}{\textbf{One-tailed binomial test statistics}:  \textbf{p-value: 0.13159};   \textbf{Confidence Interval:  0.44197 --- 1} }\\


==> mevreal502.tex <==
airlines & 0.35088 & 13539 & \textbf{0.34665} & 26718 \\
aws---price-discretized & 0.13026 & 10602 & \textbf{0.12207} & 14185 \\
chess & 0.50003 & 69 & \textbf{0.20166} & 178 \\
covertype & 0.09456 & 691 & \textbf{0.06946} & 363 \\
covpokelec & \textbf{0.06243} & 1562 & 0.07449 & 410 \\
fonts & 0.01646 & 208 & \textbf{0.00161} & 252 \\
hhar & 0.00916 & 8909 & \textbf{0.00103} & 2765 \\
kdd & \textbf{0.00073} & 163 & 0.00074 & 277 \\
localization & 0.05405 & 308 & \textbf{0.05079} & 90 \\
miniboone & \textit{\textbf{8e-05}} & 4 & \textit{\textbf{8e-05}} & 4 \\
nbaiot & 0.00096 & 58 & \textbf{0.00038} & 24 \\
nswelec & 0.15711 & 112 & \textbf{0.1462} & 105 \\
pamap2 & 0.08941 & 535 & \textbf{0.02591} & 107 \\
poker & \textbf{0.04818} & 804 & 0.09208 & 280 \\
pucrio & 0.00584 & 46 & \textbf{0.00109} & 8 \\
sensor---home-activity & 0.00279 & 595 & \textbf{0.00065} & 27 \\
sensor---CO-discretized & \textbf{0.01394} & 1950 & 0.0316 & 390 \\
skin & \textbf{0.00019} & 4 & 0.00021 & 4 \\
tnelec & \textit{\textbf{0.00315}} & 7 & \textit{\textbf{0.00315}} & 7 \\
wisdm & 0.07759 & 6204 & \textbf{0.06256} & 4205 \\
\midrule
\textbf{Unique Wins} & \multicolumn{2}{l?}{\textbf{5}} & \multicolumn{2}{l}{\textbf{13}} \\
\midrule\multicolumn{5}{l}{A \textbf{bold} error value indicates higher accuracy, and \textit{\textbf{bold italics}} indicate a tie.}\\
\multicolumn{5}{l}{\textbf{One-tailed binomial test statistics}:  \textbf{p-value: 0.04813};   \textbf{Confidence Interval:  0.50217 --- 1} }\\


==> mevreal503.tex <==
airlines & 0.33833 & 3895 & \textbf{0.33647} & 2142 \\
aws---price-discretized & 0.13031 & 10495 & \textbf{0.12231} & 13535 \\
chess & 0.03597 & 7 & \textbf{0.02683} & 7 \\
covertype & 0.08334 & 5 & \textbf{0.05854} & 13 \\
covpokelec & 0.14643 & 8 & \textbf{0.10885} & 10 \\
fonts & 0.00149 & 197 & \textbf{0.00062} & 198 \\
hhar & 0.00138 & 12 & \textbf{0.00068} & 8 \\
kdd & 0.00055 & 107 & \textbf{0.00054} & 77 \\
localization & 0.04302 & 12 & \textbf{0.03965} & 10 \\
miniboone & \textit{\textbf{8e-05}} & 4 & \textit{\textbf{8e-05}} & 4 \\
nbaiot & 0.00042 & 3 & \textbf{0.00017} & 4 \\
nswelec & 0.11343 & 22 & \textbf{0.11117} & 23 \\
pamap2 & 0.00586 & 2 & \textbf{0.00384} & 4 \\
poker & 0.18578 & 19 & \textbf{0.1385} & 23 \\
pucrio & 0.0015 & 4 & \textbf{0.00102} & 8 \\
sensor---home-activity & \textbf{0.00032} & 4 & 0.00033 & 4 \\
sensor---CO-discretized & 0.02284 & 12 & \textbf{0.01795} & 7 \\
skin & \textit{\textbf{0.00019}} & 4 & \textit{\textbf{0.00019}} & 4 \\
tnelec & \textit{\textbf{0.00291}} & 7 & \textit{\textbf{0.00291}} & 7 \\
wisdm & 0.08766 & 12 & \textbf{0.06157} & 47 \\
\midrule
\textbf{Unique Wins} & \multicolumn{2}{l?}{\textbf{1}} & \multicolumn{2}{l}{\textbf{16}} \\
\midrule\multicolumn{5}{l}{A \textbf{bold} error value indicates higher accuracy, and \textit{\textbf{bold italics}} indicate a tie.}\\
\multicolumn{5}{l}{\textbf{One-tailed binomial test statistics}:  \textbf{p-value: 0.00014};   \textbf{Confidence Interval:  0.74988 --- 1} }\\


==> mevreal504.tex <==
airlines & 0.34576 & \textbf{0.32963} \\
aws---price-discretized & \textbf{0.17592} & 0.18647 \\
chess & 0.01945 & \textbf{0.01431} \\
covertype & 0.10711 & \textbf{0.06753} \\
covpokelec & 0.18761 & \textbf{0.15185} \\
fonts & 0.006 & \textbf{0.00592} \\
hhar & 0.00148 & \textbf{0.00072} \\
kdd & 0.00041 & \textbf{4e-04} \\
localization & \textbf{0.03316} & 0.0355 \\
miniboone & \textit{\textbf{5e-05}} & \textit{\textbf{5e-05}} \\
nbaiot & 5e-05 & \textbf{4e-05} \\
nswelec & 0.12613 & \textbf{0.11209} \\
pamap2 & 0.00152 & \textbf{0.00113} \\
poker & 0.2432 & \textbf{0.20439} \\
pucrio & \textit{\textbf{0.00043}} & \textit{\textbf{0.00043}} \\
sensor---home-activity & 0.00041 & \textbf{0.00026} \\
sensor---CO-discretized & 0.00841 & \textbf{0.00767} \\
skin & \textit{\textbf{0.00013}} & \textit{\textbf{0.00013}} \\
tnelec & 0.01237 & \textbf{0.00709} \\
wisdm & 0.10829 & \textbf{0.07564} \\
\midrule
\textbf{Unique Wins} & \multicolumn{1}{l?}{\textbf{2}} & \multicolumn{1}{l}{\textbf{15}} \\
\midrule\multicolumn{3}{l}{A \textbf{bold} error value indicates higher accuracy, and \textit{\textbf{bold italics}} indicate a tie.}\\
\multicolumn{3}{l}{\textbf{One-tailed binomial test statistics}:  \textbf{p-value: 0.00117};   \textbf{Confidence Interval:  0.67381 --- 1} }\\


==> mevreal505.tex <==
airlines & \textbf{0.37629} & 9143 & 0.38124 & 9954 \\
aws---price-discretized & 0.14514 & 5590 & \textbf{0.13775} & 8145 \\
chess & 0.85683 & 15 & \textbf{0.12428} & 53 \\
covertype & 0.05509 & 111 & \textbf{0.04362} & 149 \\
covpokelec & \textbf{0.055} & 273 & 0.05874 & 284 \\
fonts & 0.00161 & 212 & \textbf{0.0016} & 224 \\
hhar & \textbf{0.01491} & 2081 & 0.02427 & 619 \\
kdd & \textbf{0.00352} & 260 & 0.00532 & 237 \\
localization & 0.0226 & 83 & \textbf{0.01916} & 98 \\
miniboone & \textit{\textbf{0.00034}} & 2 & \textit{\textbf{0.00034}} & 2 \\
nbaiot & 0.14867 & 16 & \textbf{0.1283} & 10 \\
nswelec & 0.10148 & 26 & \textbf{0.09959} & 30 \\
pamap2 & 0.62886 & 120 & \textbf{0.00756} & 35 \\
poker & 0.06793 & 158 & \textbf{0.06409} & 124 \\
pucrio & \textbf{0.00928} & 5 & 0.02264 & 4 \\
sensor---home-activity & 0.03034 & 111 & \textbf{0.0193} & 18 \\
sensor---CO-discretized & \textbf{0.01371} & 433 & 0.02023 & 107 \\
skin & \textbf{0.20743} & 4 & 0.21338 & 4 \\
tnelec & 0.00237 & 3 & \textbf{0.00159} & 3 \\
wisdm & 0.08433 & 2202 & \textbf{0.06009} & 2585 \\
\midrule
\textbf{Unique Wins} & \multicolumn{2}{l?}{\textbf{7}} & \multicolumn{2}{l}{\textbf{12}} \\
\midrule\multicolumn{5}{l}{A \textbf{bold} error value indicates higher accuracy, and \textit{\textbf{bold italics}} indicate a tie.}\\
\multicolumn{5}{l}{\textbf{One-tailed binomial test statistics}:  \textbf{p-value: 0.17964};   \textbf{Confidence Interval:  0.41806 --- 1} }\\


==> mevreal506.tex <==
airlines & 0.38917 & 4211 & \textbf{0.38814} & 3857 \\
aws---price-discretized & 0.14557 & 6529 & \textbf{0.1379} & 7852 \\
chess & 0.19479 & 8 & \textbf{0.03393} & 19 \\
covertype & 0.07792 & 33 & \textbf{0.06537} & 15 \\
covpokelec & \textbf{0.07875} & 363 & 0.11514 & 22 \\
fonts & \textbf{0.03316} & 237 & 0.03341 & 237 \\
hhar & 0.04969 & 10 & \textbf{0.00612} & 5 \\
kdd & \textbf{0.00424} & 145 & 0.00469 & 138 \\
localization & 0.04416 & 5 & \textbf{0.02743} & 6 \\
miniboone & \textit{\textbf{0.00011}} & 2 & \textit{\textbf{0.00011}} & 2 \\
nbaiot & 0.24091 & 5 & \textbf{0.12208} & 3 \\
nswelec & 0.09972 & 17 & \textbf{0.09928} & 14 \\
pamap2 & 0.13351 & 3 & \textbf{0.03107} & 3 \\
poker & \textbf{0.09119} & 339 & 0.1485 & 30 \\
pucrio & 0.00773 & 6 & \textbf{0.00763} & 5 \\
sensor---home-activity & 0.00228 & 4 & \textbf{0.00199} & 3 \\
sensor---CO-discretized & 0.08497 & 9 & \textbf{0.04265} & 4 \\
skin & \textit{\textbf{0.99942}} & 3 & \textit{\textbf{0.99942}} & 3 \\
tnelec & 0.00152 & 10 & \textbf{0.00133} & 7 \\
wisdm & 0.0782 & 480 & \textbf{0.06935} & 141 \\
\midrule
\textbf{Unique Wins} & \multicolumn{2}{l?}{\textbf{4}} & \multicolumn{2}{l}{\textbf{14}} \\
\midrule\multicolumn{5}{l}{A \textbf{bold} error value indicates higher accuracy, and \textit{\textbf{bold italics}} indicate a tie.}\\
\multicolumn{5}{l}{\textbf{One-tailed binomial test statistics}:  \textbf{p-value: 0.01544};   \textbf{Confidence Interval:  0.56112 --- 1} }\\


==> mevreal507.tex <==
airlines & \textbf{0.36174} & 9302 & 0.36964 & 9879 \\
aws---price-discretized & 0.14263 & 5432 & \textbf{0.13371} & 7627 \\
chess & 0.60293 & 14 & \textbf{0.16659} & 78 \\
covertype & 0.07985 & 154 & \textbf{0.05784} & 239 \\
covpokelec & 0.09125 & 325 & \textbf{0.08324} & 370 \\
fonts & \textit{\textbf{0.00038}} & 211 & \textit{\textbf{0.00038}} & 225 \\
hhar & 0.00152 & 2654 & \textbf{8e-04} & 1708 \\
kdd & \textbf{0.00023} & 321 & 0.00026 & 529 \\
localization & 0.04004 & 103 & \textbf{0.03828} & 95 \\
miniboone & 0.00017 & 3 & \textbf{0.00016} & 3 \\
nbaiot & \textbf{0.00354} & 36 & 0.00688 & 11 \\
nswelec & 0.13748 & 35 & \textbf{0.13211} & 36 \\
pamap2 & 0.08868 & 138 & \textbf{0.00342} & 56 \\
poker & \textbf{0.0915} & 140 & 0.10831 & 101 \\
pucrio & 0.00289 & 13 & \textbf{0.00117} & 10 \\
sensor---home-activity & 0.00206 & 176 & \textbf{0.00056} & 16 \\
sensor---CO-discretized & \textbf{0.00295} & 437 & 0.00713 & 145 \\
skin & \textit{\textbf{0.00019}} & 4 & \textit{\textbf{0.00019}} & 4 \\
tnelec & 0.00172 & 2 & \textbf{0.00159} & 8 \\
wisdm & 0.09067 & 2641 & \textbf{0.06247} & 2174 \\
\midrule
\textbf{Unique Wins} & \multicolumn{2}{l?}{\textbf{5}} & \multicolumn{2}{l}{\textbf{13}} \\
\midrule\multicolumn{5}{l}{A \textbf{bold} error value indicates higher accuracy, and \textit{\textbf{bold italics}} indicate a tie.}\\
\multicolumn{5}{l}{\textbf{One-tailed binomial test statistics}:  \textbf{p-value: 0.04813};   \textbf{Confidence Interval:  0.50217 --- 1} }\\


==> mevreal508.tex <==
airlines & \textbf{0.36173} & 9302 & 0.36963 & 9879 \\
aws---price-discretized & 0.14263 & 5432 & \textbf{0.13371} & 7627 \\
chess & 0.45517 & 14 & \textbf{0.16648} & 78 \\
covertype & 0.07985 & 154 & \textbf{0.05773} & 239 \\
covpokelec & 0.09122 & 325 & \textbf{0.08315} & 370 \\
fonts & \textit{\textbf{0.00039}} & 211 & \textit{\textbf{0.00039}} & 225 \\
hhar & 0.00152 & 2654 & \textbf{8e-04} & 1708 \\
kdd & \textbf{0.00023} & 321 & 0.00026 & 529 \\
localization & 0.04005 & 103 & \textbf{0.0383} & 95 \\
miniboone & 0.00017 & 3 & \textbf{0.00016} & 3 \\
nbaiot & \textbf{0.00355} & 36 & 0.00688 & 11 \\
nswelec & 0.13737 & 35 & \textbf{0.132} & 36 \\
pamap2 & 0.04702 & 138 & \textbf{0.00342} & 56 \\
poker & \textbf{0.09138} & 140 & 0.10831 & 101 \\
pucrio & 0.00288 & 13 & \textbf{0.00116} & 10 \\
sensor---home-activity & 0.00207 & 176 & \textbf{0.00057} & 16 \\
sensor---CO-discretized & \textbf{0.00294} & 437 & 0.00713 & 145 \\
skin & \textit{\textbf{0.00017}} & 4 & \textit{\textbf{0.00017}} & 4 \\
tnelec & 0.00172 & 2 & \textbf{0.00159} & 8 \\
wisdm & 0.09066 & 2641 & \textbf{0.06247} & 2174 \\
\midrule
\textbf{Unique Wins} & \multicolumn{2}{l?}{\textbf{5}} & \multicolumn{2}{l}{\textbf{13}} \\
\midrule\multicolumn{5}{l}{A \textbf{bold} error value indicates higher accuracy, and \textit{\textbf{bold italics}} indicate a tie.}\\
\multicolumn{5}{l}{\textbf{One-tailed binomial test statistics}:  \textbf{p-value: 0.04813};   \textbf{Confidence Interval:  0.50217 --- 1} }\\


==> mevreal509.tex <==
airlines & 0.34174 & 7253 & \textbf{0.33757} & 8791 \\
aws---price-discretized & 0.14408 & 4580 & \textbf{0.1376} & 5550 \\
chess & 0.30641 & 12 & \textbf{0.14603} & 73 \\
covertype & 0.10575 & 149 & \textbf{0.08278} & 189 \\
covpokelec & \textbf{0.09644} & 276 & 0.09676 & 258 \\
fonts & 0.00475 & 207 & \textbf{0.00148} & 212 \\
hhar & 0.01236 & 1449 & \textbf{0.00078} & 1473 \\
kdd & \textbf{0.00064} & 131 & 0.00076 & 177 \\
localization & 0.06856 & 120 & \textbf{0.04453} & 102 \\
miniboone & \textbf{0.00011} & 4 & 0.00012 & 4 \\
nbaiot & 0.03888 & 33 & \textbf{0.00332} & 24 \\
nswelec & 0.14396 & 27 & \textbf{0.13507} & 40 \\
pamap2 & 0.02624 & 128 & \textbf{0.01046} & 88 \\
poker & \textbf{0.11828} & 108 & 0.12703 & 42 \\
pucrio & 0.01445 & 12 & \textbf{0.00123} & 10 \\
sensor---home-activity & 0.00097 & 132 & \textbf{0.00039} & 25 \\
sensor---CO-discretized & \textbf{0.00816} & 310 & 0.01907 & 426 \\
skin & \textbf{0.00046} & 4 & 0.00047 & 4 \\
tnelec & \textbf{0.00241} & 2 & 0.00507 & 7 \\
wisdm & 0.10987 & 2025 & \textbf{0.08401} & 1946 \\
\midrule
\textbf{Unique Wins} & \multicolumn{2}{l?}{\textbf{7}} & \multicolumn{2}{l}{\textbf{13}} \\
\midrule\multicolumn{5}{l}{A \textbf{bold} error value indicates higher accuracy, and \textit{\textbf{bold italics}} indicate a tie.}\\
\multicolumn{5}{l}{\textbf{One-tailed binomial test statistics}:  \textbf{p-value: 0.13159};   \textbf{Confidence Interval:  0.44197 --- 1} }\\


==> mevrealshuf11.tex <==
-s (ArffFileStream -f /home/cman39/p2016030006/cman39/datasets/airlines/airlines.arff -c -1) & \textbf{0.41108} & 0.42212 \\
-s (ArffFileStream -f /home/cman39/p2016030006/cman39/datasets/aws/aws_discrete.arff -c -1) & 0.1311 & \textbf{0.12379} \\
-s (ArffFileStream -f /home/cman39/p2016030006/cman39/datasets/chess/chess.arff -c -1) & \textbf{0.62328} & 0.63585 \\
-s (ArffFileStream -f /home/cman39/p2016030006/cman39/datasets/covtype/covtype.arff) & 0.22735 & \textbf{0.22286} \\
-s (ArffFileStream -f /home/cman39/p2016030006/cman39/datasets/cpe/cpe.arff -c -1) & \textbf{0.18993} & 0.36941 \\
-s (ArffFileStream -f /home/cman39/p2016030006/cman39/datasets/fonts/fonts.arff -c 1) & \textit{\textbf{6e-04}} & \textit{\textbf{6e-04}} \\
-s (ArffFileStream -f /home/cman39/p2016030006/cman39/datasets/harpagwag/harpagwag.arff -c -1) & 0.02357 & \textbf{0.01815} \\
-s (ArffFileStream -f /home/cman39/p2016030006/cman39/datasets/kdd/kdd.arff -c -1) & 0.00063 & \textbf{0.00054} \\
-s (ArffFileStream -f /home/cman39/p2016030006/cman39/datasets/localization/localization.arff -c -1) & \textbf{0.38614} & 0.44004 \\
-s (ArffFileStream -f /home/cman39/p2016030006/cman39/datasets/miniboone/miniboone.arff -c -1) & \textbf{0.08798} & 0.09766 \\
-s (ArffFileStream -f /home/cman39/p2016030006/cman39/datasets/nbaiot/nbaiot.arff -c -1) & 0.10372 & \textbf{0.00304} \\
-s (ArffFileStream -f /home/cman39/p2016030006/cman39/datasets/nswelec/elec.arff -c -1) & \textbf{0.22097} & 0.22377 \\
-s (ArffFileStream -f /home/cman39/p2016030006/cman39/datasets/pamap2/pamap2_9subjects_.arff -c 2) & \textbf{0.33327} & 0.36266 \\
-s (ArffFileStream -f /home/cman39/p2016030006/cman39/datasets/poker/poker.arff -c -1) & \textbf{0.16436} & 0.25652 \\
-s (ArffFileStream -f /home/cman39/p2016030006/cman39/datasets/posturespucrio/pucrio.arff -c -1) & 0.04534 & \textbf{0.04214} \\
-s (ArffFileStream -f /home/cman39/p2016030006/cman39/datasets/sensor/sensor.arff -c -1) & \textbf{0.01491} & 0.02001 \\
-s (ArffFileStream -f /home/cman39/p2016030006/cman39/datasets/sensortemp2019/gassensor2019discretized.arff -c 2) & \textbf{0.12546} & 0.13818 \\
-s (ArffFileStream -f /home/cman39/p2016030006/cman39/datasets/skin/skin.arff -c -1) & 0.00529 & \textbf{0.00399} \\
-s (ArffFileStream -f /home/cman39/p2016030006/cman39/datasets/tnelec/eb.arff -c 3) & \textit{\textbf{0.00356}} & \textit{\textbf{0.00356}} \\
-s (ArffFileStream -f /home/cman39/p2016030006/cman39/datasets/wisdm/wisdm.arff -c -1) & 0.13278 & \textbf{0.11152} \\
\bottomrule &  &  \\
\begin{tabularx}{\linewidth}{Xr}
		A \textbf{bold} value indicates higher accuracy, and \textit{\textbf{bold italics}} indicate a tie.  & \textbf{Unique Wins}
		\end{tabularx} & \textbf{10} & \textbf{8} \\
\cmidrule[0.4pt](lr){2-3} &  &  \\
\begin{tabularx}{\linewidth}{Xr} The test is a one-tailed binomial test to determine the probability that the strategy in the rightmost column would achieve so many wins if wins and losses were equiprobable. & \textbf{Test Statistics} \end{tabularx} & \textbf{p-value: 0.75966} & \textbf{Confidence Interval:  0.24396 --- 1} \\


==> mevsyn11.tex <==
-s (RecurrentConceptDriftStream -x 200000 -y 200000 -z 100 -s (generators.AgrawalGenerator -f 2 -i 2) -d (generators.AgrawalGenerator -f 3 -i 3)) & 0.11408 & \textbf{0.10205} \\
-s (RecurrentConceptDriftStream -x 200000 -y 200000 -z 100 -s (generators.RandomTreeGenerator -r 1 -i 1) -d (generators.RandomTreeGenerator -r 2 -i 2)) & 0.06448 & \textbf{0.0642} \\
-s (RecurrentConceptDriftStream -x 200000 -y 200000 -z 100 -s (generators.SEAGenerator -f 2 -i 2) -d (generators.SEAGenerator -f 3 -i 3)) & 0.10672 & \textbf{0.10639} \\
-s (RecurrentConceptDriftStream -x 200000 -y 200000 -z 100 -s (generators.STAGGERGenerator -i 2 -f 2) -d (generators.STAGGERGenerator -i 3 -f 3)) & \textbf{0.00137} & 0.00141 \\
-s (generators.HyperplaneGenerator -k 10 -t 0.0001 -i 2) & \textbf{0.10714} & 0.11024 \\
-s (generators.HyperplaneGenerator -k 10 -t 0.01 -i 2) & \textbf{0.11623} & 0.11779 \\
-s (generators.HyperplaneGenerator -k 5 -t 0.0001 -i 2) & \textbf{0.10488} & 0.10881 \\
-s (generators.HyperplaneGenerator -k 5 -t 0.01 -i 2) & \textbf{0.09741} & 0.09761 \\
-s (generators.LEDGeneratorDrift -d 1 -i 2) & \textbf{0.26033} & 0.28041 \\
-s (generators.RandomRBFGeneratorDrift -s 0.0001 -k 10 -i 2 -r 2) & \textbf{0.0605} & 0.06153 \\
-s (generators.RandomRBFGeneratorDrift -s 0.0001 -k 50 -i 2 -r 2) & 0.08728 & \textbf{0.0825} \\
-s (generators.RandomRBFGeneratorDrift -s 0.001 -k 10 -i 2 -r 2) & 0.08917 & \textbf{0.08741} \\
-s (generators.RandomRBFGeneratorDrift -s 0.001 -k 50 -i 2 -r 2) & 0.18823 & \textbf{0.17382} \\
-s (generators.WaveformGeneratorDrift -d 1 -i 2 -n) & \textbf{0.14674} & 0.14862 \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 2 -n 2 -v 2 -r 2 -b 200000 -d Recurrent) & \textbf{0.08568} & 0.09068 \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 2 -v 2 -r 2 -b 200000 -d Recurrent) & \textbf{0.15231} & 0.15752 \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 3 -v 2 -r 2 -b 200000 -d Recurrent) & \textbf{0.11588} & 0.11655 \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 3 -v 3 -r 2 -b 200000 -d Recurrent) & \textbf{0.15151} & 0.16132 \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 3 -v 4 -r 2 -b 200000 -d Recurrent) & 0.21071 & \textbf{0.17869} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 3 -v 5 -r 2 -b 200000 -d Recurrent) & 0.20627 & \textbf{0.1693} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 4 -n 2 -v 2 -r 2 -b 200000 -d Recurrent) & \textbf{0.10922} & 0.11094 \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 4 -n 4 -v 4 -r 2 -b 200000 -d Recurrent) & 0.17353 & \textbf{0.12842} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 5 -n 2 -v 2 -r 2 -b 200000 -d Recurrent) & \textbf{0.11904} & 0.13362 \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 5 -n 5 -v 5 -r 2 -b 200000 -d Recurrent) & 0.13153 & \textbf{0.08684} \\
\bottomrule &  &  \\
\begin{tabularx}{\linewidth}{Xr}
		A \textbf{bold} value indicates higher accuracy, and \textit{\textbf{bold italics}} indicate a tie.  & \textbf{Unique Wins}
		\end{tabularx} & \textbf{14} & \textbf{10} \\
\cmidrule[0.4pt](lr){2-3} &  &  \\
\begin{tabularx}{\linewidth}{Xr} The test is a one-tailed binomial test to determine the probability that the strategy in the rightmost column would achieve so many wins if wins and losses were equiprobable. & \textbf{Test Statistics} \end{tabularx} & \textbf{p-value: 0.84627} & \textbf{Confidence Interval:  0.24639 --- 1} \\


==> realTables.tex <==

\begin{table}[!ht]
	
	\caption{\label{mevreal2} OzaBagADWIN
	} 
	\scriptsize
	\centering
	\makebox[0.6\textwidth]{
		
		\begin{tabular}{m{12cm}?m{1.4cm}?m{1.4cm}}
			\toprule
			\multicolumn{1}{c?}{\textbf{Streams}} &  \multicolumn{1}{m{1.4cm}}{\textbf{VFDT Base}} &
			\textbf{EFDT Base}\\
			\midrule
			\input{mevreal2.tex}
			\bottomrule
		\end{tabular}
	}
\end{table}

\begin{table}[!ht]
	
	\caption{\label{mevreal3} OnlineSmoothBoost
	} 
	\scriptsize
	\centering
	\makebox[0.6\textwidth]{
		
		\begin{tabular}{m{12cm}?m{1.4cm}?m{1.4cm}}
			\toprule
			\multicolumn{1}{c?}{\textbf{Streams}} &  \multicolumn{1}{m{1.4cm}}{\textbf{VFDT Base}} &
			\textbf{EFDT Base}\\
			\midrule
			\input{mevreal3.tex}
			\bottomrule
		\end{tabular}
	}
\end{table}


\begin{table}[!ht]
	
	\caption{\label{mevreal4} OzaBoost
	} 
	\scriptsize
	\centering
	\makebox[0.6\textwidth]{
		
		\begin{tabular}{m{12cm}?m{1.4cm}?m{1.4cm}}
			\toprule
			\multicolumn{1}{c?}{\textbf{Streams}} &  \multicolumn{1}{m{1.4cm}}{\textbf{VFDT Base}} &
			\textbf{EFDT Base}\\
			\midrule
			\input{mevreal4.tex}
			\bottomrule
		\end{tabular}
	}
\end{table}


\begin{table}[!ht]
	
	\caption{\label{mevreal5} LevBagNoADWIN
	} 
	\scriptsize
	\centering
	\makebox[0.6\textwidth]{
		
		\begin{tabular}{m{12cm}?m{1.4cm}?m{1.4cm}}
			\toprule
			\multicolumn{1}{c?}{\textbf{Streams}} &  \multicolumn{1}{m{1.4cm}}{\textbf{VFDT Base}} &
			\textbf{EFDT Base}\\
			\midrule
			\input{mevreal5.tex}
			\bottomrule
		\end{tabular}
	}
\end{table}





\begin{table}[!ht]
	
	\caption{\label{mevreal6} ARF Optimised Parametrization
	} 
	\scriptsize
	\centering
	\makebox[0.6\textwidth]{
		
		\begin{tabular}{m{12cm}?m{1.4cm}?m{1.4cm}}
			\toprule
			\multicolumn{1}{c?}{\textbf{Streams}} &  \multicolumn{1}{m{1.4cm}}{\textbf{VFDT Base}} &
			\textbf{EFDT Base}\\
			\midrule
			\input{mevreal6.tex}
			\bottomrule
		\end{tabular}
	}
\end{table}

\begin{table}[!ht]
	
	\caption{\label{mevreal7} OzaBoostADWIN
	} 
	\scriptsize
	\centering
	\makebox[0.6\textwidth]{
		
		\begin{tabular}{m{12cm}?m{1.4cm}?m{1.4cm}}
			\toprule
			\multicolumn{1}{c?}{\textbf{Streams}} &  \multicolumn{1}{m{1.4cm}}{\textbf{VFDT Base}} &
			\textbf{EFDT Base}\\
			\midrule
			\input{mevreal7.tex}
			\bottomrule
		\end{tabular}
	}
\end{table}



\begin{table}[!ht]
	
	\caption{\label{mevreal8} Plain single learners (no ensemble)
	} 
	\scriptsize
	\centering
	\makebox[0.6\textwidth]{
		
		\begin{tabular}{m{12cm}?m{1.4cm}?m{1.4cm}}
			\toprule
			\multicolumn{1}{c?}{\textbf{Streams}} &  \multicolumn{1}{m{1.4cm}}{\textbf{VFDT Base}} &
			\textbf{EFDT Base}\\
			\midrule
			\input{mevreal8.tex}
			\bottomrule
		\end{tabular}
	}
\end{table}


\begin{table}[!ht]
	
	\caption{\label{mevreal9} OzaBag
	} 
	\scriptsize
	\centering
	\makebox[0.6\textwidth]{
		
		\begin{tabular}{m{12cm}?m{1.4cm}?m{1.4cm}}
			\toprule
			\multicolumn{1}{c?}{\textbf{Streams}} &  \multicolumn{1}{m{1.4cm}}{\textbf{VFDT Base}} &
			\textbf{EFDT Base}\\
			\midrule
			\input{mevreal9.tex}
			\bottomrule
		\end{tabular}
	}
\end{table}

\begin{table}[!ht]
	
	\caption{\label{mevreal10} ADOB
	} 
	\scriptsize
	\centering
	\makebox[0.6\textwidth]{
		
		\begin{tabular}{m{12cm}?m{1.4cm}?m{1.4cm}}
			\toprule
			\multicolumn{1}{c?}{\textbf{Streams}} &  \multicolumn{1}{m{1.4cm}}{\textbf{VFDT Base}} &
			\textbf{EFDT Base}\\
			\midrule
			\input{mevreal10.tex}
			\bottomrule
		\end{tabular}
	}
\end{table}


\begin{table}[!ht]
	
	\caption{\label{mevreal11} LevBag
	} 
	\scriptsize
	\centering
	\makebox[0.6\textwidth]{
		
		\begin{tabular}{m{12cm}?m{1.4cm}?m{1.4cm}}
			\toprule
			\multicolumn{1}{c?}{\textbf{Streams}} &  \multicolumn{1}{m{1.4cm}}{\textbf{VFDT Base}} &
			\textbf{EFDT Base}\\
			\midrule
			\input{mevreal11.tex}
			\bottomrule
		\end{tabular}
	}
	
\end{table}



==> table1.tex <==
-s (RecurrentConceptDriftStream -x 200000 -y 200000 -z 100 -s (generators.AgrawalGenerator -f 2 -i 2) -d (generators.AgrawalGenerator -f 3 -i 3)) & 0.13645 & \textbf{0.13643} \\
-s (RecurrentConceptDriftStream -x 200000 -y 200000 -z 100 -s (generators.RandomTreeGenerator -r 1 -i 1) -d (generators.RandomTreeGenerator -r 2 -i 2)) & \textbf{0.10104} & 0.10615 \\
-s (RecurrentConceptDriftStream -x 200000 -y 200000 -z 100 -s (generators.SEAGenerator -f 2 -i 2) -d (generators.SEAGenerator -f 3 -i 3)) & 0.12579 & \textbf{0.12538} \\
-s (RecurrentConceptDriftStream -x 200000 -y 200000 -z 100 -s (generators.STAGGERGenerator -i 2 -f 2) -d (generators.STAGGERGenerator -i 3 -f 3)) & 0.00215 & \textbf{0.00136} \\
-s (generators.HyperplaneGenerator -k 10 -t 0.0001 -i 2) & 0.10801 & \textbf{0.10576} \\
-s (generators.HyperplaneGenerator -k 10 -t 0.001 -i 2) & 0.11934 & \textbf{0.11606} \\
-s (generators.HyperplaneGenerator -k 10 -t 0.01 -i 2) & 0.1198 & \textbf{0.11681} \\
-s (generators.HyperplaneGenerator -k 5 -t 0.0001 -i 2) & 0.10588 & \textbf{0.10412} \\
-s (generators.HyperplaneGenerator -k 5 -t 0.001 -i 2) & 0.11254 & \textbf{0.10947} \\
-s (generators.HyperplaneGenerator -k 5 -t 0.01 -i 2) & 0.10767 & \textbf{0.1047} \\
-s (generators.LEDGeneratorDrift -d 1 -i 2) & 0.26137 & \textbf{0.26123} \\
-s (generators.LEDGeneratorDrift -d 3 -i 2) & 0.26137 & \textbf{0.26123} \\
-s (generators.LEDGeneratorDrift -d 5 -i 2) & 0.26137 & \textbf{0.26123} \\
-s (generators.LEDGeneratorDrift -d 7 -i 2) & 0.26137 & \textbf{0.26123} \\
-s (generators.RandomRBFGeneratorDrift -s 0.0001 -k 10 -i 2 -r 2) & 0.13508 & \textbf{0.13109} \\
-s (generators.RandomRBFGeneratorDrift -s 0.0001 -k 50 -i 2 -r 2) & 0.19549 & \textbf{0.18094} \\
-s (generators.RandomRBFGeneratorDrift -s 0.001 -k 10 -i 2 -r 2) & 0.16636 & \textbf{0.16503} \\
-s (generators.RandomRBFGeneratorDrift -s 0.001 -k 50 -i 2 -r 2) & 0.33926 & \textbf{0.32535} \\
-s (generators.WaveformGeneratorDrift -d 1 -i 2 -n) & 0.16279 & \textbf{0.16251} \\
-s (generators.WaveformGeneratorDrift -d 3 -i 2 -n) & 0.16279 & \textbf{0.16251} \\
-s (generators.WaveformGeneratorDrift -d 5 -i 2 -n) & 0.16279 & \textbf{0.16251} \\
-s (generators.WaveformGeneratorDrift -d 7 -i 2 -n) & 0.16279 & \textbf{0.16251} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 2 -n 2 -v 2 -r 2 -b 200000 -d Recurrent) & 0.00185 & \textbf{7e-04} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 2 -v 2 -r 2 -b 200000 -d Recurrent) & 0.0016 & \textbf{0.00056} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 3 -v 2 -r 2 -b 200000 -d Recurrent) & 0.00252 & \textbf{0.00144} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 3 -v 3 -r 2 -b 200000 -d Recurrent) & \textbf{0.00425} & 0.00475 \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 3 -v 4 -r 2 -b 200000 -d Recurrent) & \textbf{0.01212} & 0.01389 \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 3 -v 5 -r 2 -b 200000 -d Recurrent) & \textbf{0.01687} & 0.01978 \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 4 -n 2 -v 2 -r 2 -b 200000 -d Recurrent) & 0.00177 & \textbf{0.00049} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 4 -n 4 -v 4 -r 2 -b 200000 -d Recurrent) & \textbf{0.06662} & 0.07347 \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 5 -n 2 -v 2 -r 2 -b 200000 -d Recurrent) & 0.00177 & \textbf{0.00037} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 5 -n 5 -v 5 -r 2 -b 200000 -d Recurrent) & \textbf{0.34892} & 0.35605 \\
\bottomrule &  &  \\
\begin{tabularx}{\linewidth}{Xr}
		A \textbf{bold} value indicates higher accuracy, and \textit{\textbf{bold italics}} indicate a tie.  & \textbf{Unique Wins}
		\end{tabularx} & \textbf{6} & \textbf{26} \\
\cmidrule[0.4pt](lr){2-3} &  &  \\
\begin{tabularx}{\linewidth}{Xr} The test is a simple binomial test to determine whether the strategy in the rightmost 
             column is likely to have an equal number of ``wins'' as the strategy being compared against on the left. & \textbf{Test Statistics} \end{tabularx} & \textbf{p-value: 0.00027} & \textbf{Confidence Interval:  0.66313 --- 1} \\


==> table10.tex <==
-s (RecurrentConceptDriftStream -x 200000 -y 200000 -z 100 -s (generators.AgrawalGenerator -f 2 -i 2) -d (generators.AgrawalGenerator -f 3 -i 3)) & 0.13098 & \textbf{0.12793} \\
-s (RecurrentConceptDriftStream -x 200000 -y 200000 -z 100 -s (generators.RandomTreeGenerator -r 1 -i 1) -d (generators.RandomTreeGenerator -r 2 -i 2)) & \textbf{0.0994} & 0.12227 \\
-s (RecurrentConceptDriftStream -x 200000 -y 200000 -z 100 -s (generators.SEAGenerator -f 2 -i 2) -d (generators.SEAGenerator -f 3 -i 3)) & \textbf{0.11224} & 0.11853 \\
-s (RecurrentConceptDriftStream -x 200000 -y 200000 -z 100 -s (generators.STAGGERGenerator -i 2 -f 2) -d (generators.STAGGERGenerator -i 3 -f 3)) & \textbf{0.00187} & 0.00188 \\
-s (generators.HyperplaneGenerator -k 10 -t 0.0001 -i 2) & 0.11936 & \textbf{0.11644} \\
-s (generators.HyperplaneGenerator -k 10 -t 0.001 -i 2) & 0.13425 & \textbf{0.1241} \\
-s (generators.HyperplaneGenerator -k 10 -t 0.01 -i 2) & 0.13181 & \textbf{0.12509} \\
-s (generators.HyperplaneGenerator -k 5 -t 0.0001 -i 2) & 0.13868 & \textbf{0.11753} \\
-s (generators.HyperplaneGenerator -k 5 -t 0.001 -i 2) & \textbf{0.11149} & 0.11526 \\
-s (generators.HyperplaneGenerator -k 5 -t 0.01 -i 2) & \textbf{0.10533} & 0.10867 \\
-s (generators.LEDGeneratorDrift -d 1 -i 2) & \textbf{0.26118} & 0.26124 \\
-s (generators.LEDGeneratorDrift -d 3 -i 2) & \textbf{0.26118} & 0.26124 \\
-s (generators.LEDGeneratorDrift -d 5 -i 2) & \textbf{0.26118} & 0.26124 \\
-s (generators.LEDGeneratorDrift -d 7 -i 2) & \textbf{0.26118} & 0.26124 \\
-s (generators.RandomRBFGeneratorDrift -s 0.0001 -k 10 -i 2 -r 2) & 0.13354 & \textbf{0.12037} \\
-s (generators.RandomRBFGeneratorDrift -s 0.0001 -k 50 -i 2 -r 2) & 0.18126 & \textbf{0.18017} \\
-s (generators.RandomRBFGeneratorDrift -s 0.001 -k 10 -i 2 -r 2) & 0.19556 & \textbf{0.15522} \\
-s (generators.RandomRBFGeneratorDrift -s 0.001 -k 50 -i 2 -r 2) & \textbf{0.32677} & 0.32757 \\
-s (generators.WaveformGeneratorDrift -d 1 -i 2 -n) & 0.17888 & \textbf{0.17118} \\
-s (generators.WaveformGeneratorDrift -d 3 -i 2 -n) & 0.17888 & \textbf{0.17118} \\
-s (generators.WaveformGeneratorDrift -d 5 -i 2 -n) & 0.17888 & \textbf{0.17118} \\
-s (generators.WaveformGeneratorDrift -d 7 -i 2 -n) & 0.17887 & \textbf{0.17118} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 2 -n 2 -v 2 -r 2 -b 200000 -d Recurrent) & \textbf{0.00065} & 0.00068 \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 2 -v 2 -r 2 -b 200000 -d Recurrent) & 0.00068 & \textbf{0.00062} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 3 -v 2 -r 2 -b 200000 -d Recurrent) & 0.00167 & \textbf{0.00122} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 3 -v 3 -r 2 -b 200000 -d Recurrent) & 0.00642 & \textbf{0.00307} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 3 -v 4 -r 2 -b 200000 -d Recurrent) & 0.01252 & \textbf{0.0093} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 3 -v 5 -r 2 -b 200000 -d Recurrent) & \textbf{0.01473} & 0.01475 \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 4 -n 2 -v 2 -r 2 -b 200000 -d Recurrent) & \textbf{0.00069} & 0.00073 \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 4 -n 4 -v 4 -r 2 -b 200000 -d Recurrent) & \textbf{0.05099} & 0.05314 \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 5 -n 2 -v 2 -r 2 -b 200000 -d Recurrent) & 0.00079 & \textbf{0.00078} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 5 -n 5 -v 5 -r 2 -b 200000 -d Recurrent) & \textbf{0.28127} & 0.28637 \\
\bottomrule &  &  \\
\begin{tabularx}{\linewidth}{Xr}
		A \textbf{bold} value indicates higher accuracy, and \textit{\textbf{bold italics}} indicate a tie.  & \textbf{Unique Wins}
		\end{tabularx} & \textbf{15} & \textbf{17} \\
\cmidrule[0.4pt](lr){2-3} &  &  \\
\begin{tabularx}{\linewidth}{Xr} The test is a simple binomial test to determine whether the strategy in the rightmost 
             column is likely to have an equal number of ``wins'' as the strategy being compared against on the left. & \textbf{Test Statistics} \end{tabularx} & \textbf{p-value: 0.43003} & \textbf{Confidence Interval:  0.37339 --- 1} \\


==> table101.tex <==
-s (RecurrentConceptDriftStream -x 200000 -y 200000 -z 100 -s (generators.AgrawalGenerator -f 2 -i 2) -d (generators.AgrawalGenerator -f 3 -i 3)) & 0.20846 & \textbf{0.19894} \\
-s (RecurrentConceptDriftStream -x 200000 -y 200000 -z 100 -s (generators.RandomTreeGenerator -r 1 -i 1) -d (generators.RandomTreeGenerator -r 2 -i 2)) & 0.22404 & \textbf{0.22151} \\
-s (RecurrentConceptDriftStream -x 200000 -y 200000 -z 100 -s (generators.SEAGenerator -f 2 -i 2) -d (generators.SEAGenerator -f 3 -i 3)) & 0.15251 & \textbf{0.15239} \\
-s (RecurrentConceptDriftStream -x 200000 -y 200000 -z 100 -s (generators.STAGGERGenerator -i 2 -f 2) -d (generators.STAGGERGenerator -i 3 -f 3)) & 0.1882 & \textbf{0.00699} \\
-s (generators.HyperplaneGenerator -k 10 -t 0.0001 -i 2) & 0.11566 & \textbf{0.11455} \\
-s (generators.HyperplaneGenerator -k 10 -t 0.001 -i 2) & 0.16785 & \textbf{0.16458} \\
-s (generators.HyperplaneGenerator -k 10 -t 0.01 -i 2) & 0.1713 & \textbf{0.1685} \\
-s (generators.HyperplaneGenerator -k 5 -t 0.0001 -i 2) & 0.1074 & \textbf{0.10714} \\
-s (generators.HyperplaneGenerator -k 5 -t 0.001 -i 2) & 0.16309 & \textbf{0.16005} \\
-s (generators.HyperplaneGenerator -k 5 -t 0.01 -i 2) & 0.17108 & \textbf{0.16579} \\
-s (generators.LEDGeneratorDrift -d 1 -i 2) & \textit{\textbf{0.26093}} & \textit{\textbf{0.26093}} \\
-s (generators.LEDGeneratorDrift -d 3 -i 2) & \textit{\textbf{0.26093}} & \textit{\textbf{0.26093}} \\
-s (generators.LEDGeneratorDrift -d 5 -i 2) & \textit{\textbf{0.26093}} & \textit{\textbf{0.26093}} \\
-s (generators.LEDGeneratorDrift -d 7 -i 2) & \textit{\textbf{0.26093}} & \textit{\textbf{0.26093}} \\
-s (generators.RandomRBFGeneratorDrift -s 0.0001 -k 10 -i 2 -r 2) & 0.11462 & \textbf{0.11381} \\
-s (generators.RandomRBFGeneratorDrift -s 0.0001 -k 50 -i 2 -r 2) & 0.2858 & \textbf{0.28486} \\
-s (generators.RandomRBFGeneratorDrift -s 0.001 -k 10 -i 2 -r 2) & 0.13821 & \textbf{0.1377} \\
-s (generators.RandomRBFGeneratorDrift -s 0.001 -k 50 -i 2 -r 2) & 0.40874 & \textbf{0.40583} \\
-s (generators.WaveformGeneratorDrift -d 1 -i 2 -n) & \textit{\textbf{0.16284}} & \textit{\textbf{0.16284}} \\
-s (generators.WaveformGeneratorDrift -d 3 -i 2 -n) & \textit{\textbf{0.16284}} & \textit{\textbf{0.16284}} \\
-s (generators.WaveformGeneratorDrift -d 5 -i 2 -n) & \textit{\textbf{0.16284}} & \textit{\textbf{0.16284}} \\
-s (generators.WaveformGeneratorDrift -d 7 -i 2 -n) & \textit{\textbf{0.16284}} & \textit{\textbf{0.16284}} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 2 -n 2 -v 2 -r 2 -b 200000 -d Recurrent) & 0.35403 & \textbf{0.00261} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 2 -v 2 -r 2 -b 200000 -d Recurrent) & 0.37862 & \textbf{0.00325} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 3 -v 2 -r 2 -b 200000 -d Recurrent) & 0.3504 & \textbf{0.01316} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 3 -v 3 -r 2 -b 200000 -d Recurrent) & 0.36505 & \textbf{0.0582} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 3 -v 4 -r 2 -b 200000 -d Recurrent) & 0.39687 & \textbf{0.15073} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 3 -v 5 -r 2 -b 200000 -d Recurrent) & 0.39622 & \textbf{0.23007} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 4 -n 2 -v 2 -r 2 -b 200000 -d Recurrent) & 0.33416 & \textbf{0.00959} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 4 -n 4 -v 4 -r 2 -b 200000 -d Recurrent) & 0.40671 & \textbf{0.34738} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 5 -n 2 -v 2 -r 2 -b 200000 -d Recurrent) & 0.3309 & \textbf{0.00937} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 5 -n 5 -v 5 -r 2 -b 200000 -d Recurrent) & 0.46461 & \textbf{0.46352} \\
\bottomrule &  &  \\
\begin{tabularx}{\linewidth}{Xr}
		A \textbf{bold} value indicates higher accuracy, and \textit{\textbf{bold italics}} indicate a tie.  & \textbf{Unique Wins}
		\end{tabularx} & \textbf{0} & \textbf{24} \\
\cmidrule[0.4pt](lr){2-3} &  &  \\
\begin{tabularx}{\linewidth}{Xr} The test is a simple binomial test to determine whether the strategy in the rightmost 
             column is likely to have an equal number of ``wins'' as the strategy being compared against on the left. & \textbf{Test Statistics} \end{tabularx} & \textbf{p-value: 0} & \textbf{Confidence Interval:  0.88265 --- 1} \\


==> table102.tex <==
-s (RecurrentConceptDriftStream -x 200000 -y 200000 -z 100 -s (generators.AgrawalGenerator -f 2 -i 2) -d (generators.AgrawalGenerator -f 3 -i 3)) & 0.20846 & \textbf{0.20774} \\
-s (RecurrentConceptDriftStream -x 200000 -y 200000 -z 100 -s (generators.RandomTreeGenerator -r 1 -i 1) -d (generators.RandomTreeGenerator -r 2 -i 2)) & 0.22404 & \textbf{0.22367} \\
-s (RecurrentConceptDriftStream -x 200000 -y 200000 -z 100 -s (generators.SEAGenerator -f 2 -i 2) -d (generators.SEAGenerator -f 3 -i 3)) & 0.15251 & \textbf{0.15228} \\
-s (RecurrentConceptDriftStream -x 200000 -y 200000 -z 100 -s (generators.STAGGERGenerator -i 2 -f 2) -d (generators.STAGGERGenerator -i 3 -f 3)) & \textit{\textbf{0.1882}} & \textit{\textbf{0.1882}} \\
-s (generators.HyperplaneGenerator -k 10 -t 0.0001 -i 2) & \textbf{0.11566} & 0.11576 \\
-s (generators.HyperplaneGenerator -k 10 -t 0.001 -i 2) & \textbf{0.16785} & 0.1681 \\
-s (generators.HyperplaneGenerator -k 10 -t 0.01 -i 2) & \textbf{0.1713} & 0.17202 \\
-s (generators.HyperplaneGenerator -k 5 -t 0.0001 -i 2) & \textbf{0.1074} & 0.10745 \\
-s (generators.HyperplaneGenerator -k 5 -t 0.001 -i 2) & 0.16309 & \textbf{0.16251} \\
-s (generators.HyperplaneGenerator -k 5 -t 0.01 -i 2) & \textbf{0.17108} & 0.17114 \\
-s (generators.LEDGeneratorDrift -d 1 -i 2) & 0.26093 & \textbf{0.26086} \\
-s (generators.LEDGeneratorDrift -d 3 -i 2) & 0.26093 & \textbf{0.26086} \\
-s (generators.LEDGeneratorDrift -d 5 -i 2) & 0.26093 & \textbf{0.26086} \\
-s (generators.LEDGeneratorDrift -d 7 -i 2) & 0.26093 & \textbf{0.26086} \\
-s (generators.RandomRBFGeneratorDrift -s 0.0001 -k 10 -i 2 -r 2) & 0.11462 & \textbf{0.11446} \\
-s (generators.RandomRBFGeneratorDrift -s 0.0001 -k 50 -i 2 -r 2) & 0.2858 & \textbf{0.28565} \\
-s (generators.RandomRBFGeneratorDrift -s 0.001 -k 10 -i 2 -r 2) & \textbf{0.13821} & 0.13867 \\
-s (generators.RandomRBFGeneratorDrift -s 0.001 -k 50 -i 2 -r 2) & \textbf{0.40874} & 0.40887 \\
-s (generators.WaveformGeneratorDrift -d 1 -i 2 -n) & 0.16284 & \textbf{0.16276} \\
-s (generators.WaveformGeneratorDrift -d 3 -i 2 -n) & 0.16284 & \textbf{0.16276} \\
-s (generators.WaveformGeneratorDrift -d 5 -i 2 -n) & 0.16284 & \textbf{0.16276} \\
-s (generators.WaveformGeneratorDrift -d 7 -i 2 -n) & 0.16284 & \textbf{0.16276} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 2 -n 2 -v 2 -r 2 -b 200000 -d Recurrent) & 0.35403 & \textbf{0.35402} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 2 -v 2 -r 2 -b 200000 -d Recurrent) & \textit{\textbf{0.37862}} & \textit{\textbf{0.37862}} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 3 -v 2 -r 2 -b 200000 -d Recurrent) & \textbf{0.3504} & 0.35104 \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 3 -v 3 -r 2 -b 200000 -d Recurrent) & 0.36505 & \textbf{0.36503} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 3 -v 4 -r 2 -b 200000 -d Recurrent) & 0.39687 & \textbf{0.39678} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 3 -v 5 -r 2 -b 200000 -d Recurrent) & \textbf{0.39622} & 0.39635 \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 4 -n 2 -v 2 -r 2 -b 200000 -d Recurrent) & \textit{\textbf{0.33416}} & \textit{\textbf{0.33416}} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 4 -n 4 -v 4 -r 2 -b 200000 -d Recurrent) & 0.40671 & \textbf{0.40632} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 5 -n 2 -v 2 -r 2 -b 200000 -d Recurrent) & \textbf{0.3309} & 0.3312 \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 5 -n 5 -v 5 -r 2 -b 200000 -d Recurrent) & 0.46461 & \textbf{0.46106} \\
\bottomrule &  &  \\
\begin{tabularx}{\linewidth}{Xr}
		A \textbf{bold} value indicates higher accuracy, and \textit{\textbf{bold italics}} indicate a tie.  & \textbf{Unique Wins}
		\end{tabularx} & \textbf{10} & \textbf{19} \\
\cmidrule[0.4pt](lr){2-3} &  &  \\
\begin{tabularx}{\linewidth}{Xr} The test is a simple binomial test to determine whether the strategy in the rightmost 
             column is likely to have an equal number of ``wins'' as the strategy being compared against on the left. & \textbf{Test Statistics} \end{tabularx} & \textbf{p-value: 0.06802} & \textbf{Confidence Interval:  0.48573 --- 1} \\


==> table103.tex <==
-s (RecurrentConceptDriftStream -x 200000 -y 200000 -z 100 -s (generators.AgrawalGenerator -f 2 -i 2) -d (generators.AgrawalGenerator -f 3 -i 3)) & 0.20846 & \textbf{0.2078} \\
-s (RecurrentConceptDriftStream -x 200000 -y 200000 -z 100 -s (generators.RandomTreeGenerator -r 1 -i 1) -d (generators.RandomTreeGenerator -r 2 -i 2)) & 0.22404 & \textbf{0.22403} \\
-s (RecurrentConceptDriftStream -x 200000 -y 200000 -z 100 -s (generators.SEAGenerator -f 2 -i 2) -d (generators.SEAGenerator -f 3 -i 3)) & \textbf{0.15251} & 0.15253 \\
-s (RecurrentConceptDriftStream -x 200000 -y 200000 -z 100 -s (generators.STAGGERGenerator -i 2 -f 2) -d (generators.STAGGERGenerator -i 3 -f 3)) & \textit{\textbf{0.1882}} & \textit{\textbf{0.1882}} \\
-s (generators.HyperplaneGenerator -k 10 -t 0.0001 -i 2) & 0.11566 & \textbf{0.11565} \\
-s (generators.HyperplaneGenerator -k 10 -t 0.001 -i 2) & \textbf{0.16785} & 0.16801 \\
-s (generators.HyperplaneGenerator -k 10 -t 0.01 -i 2) & \textbf{0.1713} & 0.17145 \\
-s (generators.HyperplaneGenerator -k 5 -t 0.0001 -i 2) & \textbf{0.1074} & 0.10744 \\
-s (generators.HyperplaneGenerator -k 5 -t 0.001 -i 2) & 0.16309 & \textbf{0.16287} \\
-s (generators.HyperplaneGenerator -k 5 -t 0.01 -i 2) & 0.17108 & \textbf{0.17075} \\
-s (generators.LEDGeneratorDrift -d 1 -i 2) & \textit{\textbf{0.26093}} & \textit{\textbf{0.26093}} \\
-s (generators.LEDGeneratorDrift -d 3 -i 2) & \textit{\textbf{0.26093}} & \textit{\textbf{0.26093}} \\
-s (generators.LEDGeneratorDrift -d 5 -i 2) & \textit{\textbf{0.26093}} & \textit{\textbf{0.26093}} \\
-s (generators.LEDGeneratorDrift -d 7 -i 2) & \textit{\textbf{0.26093}} & \textit{\textbf{0.26093}} \\
-s (generators.RandomRBFGeneratorDrift -s 0.0001 -k 10 -i 2 -r 2) & 0.11462 & \textbf{0.11458} \\
-s (generators.RandomRBFGeneratorDrift -s 0.0001 -k 50 -i 2 -r 2) & \textbf{0.2858} & 0.2862 \\
-s (generators.RandomRBFGeneratorDrift -s 0.001 -k 10 -i 2 -r 2) & \textbf{0.13821} & 0.13852 \\
-s (generators.RandomRBFGeneratorDrift -s 0.001 -k 50 -i 2 -r 2) & 0.40874 & \textbf{0.40853} \\
-s (generators.WaveformGeneratorDrift -d 1 -i 2 -n) & 0.16284 & \textbf{0.16274} \\
-s (generators.WaveformGeneratorDrift -d 3 -i 2 -n) & 0.16284 & \textbf{0.16274} \\
-s (generators.WaveformGeneratorDrift -d 5 -i 2 -n) & 0.16284 & \textbf{0.16274} \\
-s (generators.WaveformGeneratorDrift -d 7 -i 2 -n) & 0.16284 & \textbf{0.16274} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 2 -n 2 -v 2 -r 2 -b 200000 -d Recurrent) & \textit{\textbf{0.35403}} & \textit{\textbf{0.35403}} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 2 -v 2 -r 2 -b 200000 -d Recurrent) & \textit{\textbf{0.37862}} & \textit{\textbf{0.37862}} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 3 -v 2 -r 2 -b 200000 -d Recurrent) & \textit{\textbf{0.3504}} & \textit{\textbf{0.3504}} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 3 -v 3 -r 2 -b 200000 -d Recurrent) & \textit{\textbf{0.36505}} & \textit{\textbf{0.36505}} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 3 -v 4 -r 2 -b 200000 -d Recurrent) & \textit{\textbf{0.39687}} & \textit{\textbf{0.39687}} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 3 -v 5 -r 2 -b 200000 -d Recurrent) & \textit{\textbf{0.39622}} & \textit{\textbf{0.39622}} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 4 -n 2 -v 2 -r 2 -b 200000 -d Recurrent) & \textit{\textbf{0.33416}} & \textit{\textbf{0.33416}} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 4 -n 4 -v 4 -r 2 -b 200000 -d Recurrent) & \textit{\textbf{0.40671}} & \textit{\textbf{0.40671}} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 5 -n 2 -v 2 -r 2 -b 200000 -d Recurrent) & \textit{\textbf{0.3309}} & \textit{\textbf{0.3309}} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 5 -n 5 -v 5 -r 2 -b 200000 -d Recurrent) & \textit{\textbf{0.46461}} & \textit{\textbf{0.46461}} \\
\bottomrule &  &  \\
\begin{tabularx}{\linewidth}{Xr}
		A \textbf{bold} value indicates higher accuracy, and \textit{\textbf{bold italics}} indicate a tie.  & \textbf{Unique Wins}
		\end{tabularx} & \textbf{6} & \textbf{11} \\
\cmidrule[0.4pt](lr){2-3} &  &  \\
\begin{tabularx}{\linewidth}{Xr} The test is a simple binomial test to determine whether the strategy in the rightmost 
             column is likely to have an equal number of ``wins'' as the strategy being compared against on the left. & \textbf{Test Statistics} \end{tabularx} & \textbf{p-value: 0.16615} & \textbf{Confidence Interval:  0.41971 --- 1} \\


==> table104.tex <==
-s (RecurrentConceptDriftStream -x 200000 -y 200000 -z 100 -s (generators.AgrawalGenerator -f 2 -i 2) -d (generators.AgrawalGenerator -f 3 -i 3)) & 0.20846 & \textbf{0.1977} \\
-s (RecurrentConceptDriftStream -x 200000 -y 200000 -z 100 -s (generators.RandomTreeGenerator -r 1 -i 1) -d (generators.RandomTreeGenerator -r 2 -i 2)) & 0.22404 & \textbf{0.22123} \\
-s (RecurrentConceptDriftStream -x 200000 -y 200000 -z 100 -s (generators.SEAGenerator -f 2 -i 2) -d (generators.SEAGenerator -f 3 -i 3)) & 0.15251 & \textbf{0.15237} \\
-s (RecurrentConceptDriftStream -x 200000 -y 200000 -z 100 -s (generators.STAGGERGenerator -i 2 -f 2) -d (generators.STAGGERGenerator -i 3 -f 3)) & 0.1882 & \textbf{0.00699} \\
-s (generators.HyperplaneGenerator -k 10 -t 0.0001 -i 2) & 0.11566 & \textbf{0.11464} \\
-s (generators.HyperplaneGenerator -k 10 -t 0.001 -i 2) & 0.16785 & \textbf{0.16436} \\
-s (generators.HyperplaneGenerator -k 10 -t 0.01 -i 2) & 0.1713 & \textbf{0.16945} \\
-s (generators.HyperplaneGenerator -k 5 -t 0.0001 -i 2) & 0.1074 & \textbf{0.10723} \\
-s (generators.HyperplaneGenerator -k 5 -t 0.001 -i 2) & 0.16309 & \textbf{0.15871} \\
-s (generators.HyperplaneGenerator -k 5 -t 0.01 -i 2) & 0.17108 & \textbf{0.16479} \\
-s (generators.LEDGeneratorDrift -d 1 -i 2) & 0.26093 & \textbf{0.26087} \\
-s (generators.LEDGeneratorDrift -d 3 -i 2) & 0.26093 & \textbf{0.26087} \\
-s (generators.LEDGeneratorDrift -d 5 -i 2) & 0.26093 & \textbf{0.26087} \\
-s (generators.LEDGeneratorDrift -d 7 -i 2) & 0.26093 & \textbf{0.26087} \\
-s (generators.RandomRBFGeneratorDrift -s 0.0001 -k 10 -i 2 -r 2) & 0.11462 & \textbf{0.11331} \\
-s (generators.RandomRBFGeneratorDrift -s 0.0001 -k 50 -i 2 -r 2) & 0.2858 & \textbf{0.28356} \\
-s (generators.RandomRBFGeneratorDrift -s 0.001 -k 10 -i 2 -r 2) & 0.13821 & \textbf{0.13803} \\
-s (generators.RandomRBFGeneratorDrift -s 0.001 -k 50 -i 2 -r 2) & 0.40874 & \textbf{0.40593} \\
-s (generators.WaveformGeneratorDrift -d 1 -i 2 -n) & 0.16284 & \textbf{0.16271} \\
-s (generators.WaveformGeneratorDrift -d 3 -i 2 -n) & 0.16284 & \textbf{0.16271} \\
-s (generators.WaveformGeneratorDrift -d 5 -i 2 -n) & 0.16284 & \textbf{0.16271} \\
-s (generators.WaveformGeneratorDrift -d 7 -i 2 -n) & 0.16284 & \textbf{0.16271} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 2 -n 2 -v 2 -r 2 -b 200000 -d Recurrent) & 0.35403 & \textbf{0.00263} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 2 -v 2 -r 2 -b 200000 -d Recurrent) & 0.37862 & \textbf{0.00328} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 3 -v 2 -r 2 -b 200000 -d Recurrent) & 0.3504 & \textbf{0.01349} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 3 -v 3 -r 2 -b 200000 -d Recurrent) & 0.36505 & \textbf{0.05837} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 3 -v 4 -r 2 -b 200000 -d Recurrent) & 0.39687 & \textbf{0.15038} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 3 -v 5 -r 2 -b 200000 -d Recurrent) & 0.39622 & \textbf{0.23056} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 4 -n 2 -v 2 -r 2 -b 200000 -d Recurrent) & 0.33416 & \textbf{0.0096} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 4 -n 4 -v 4 -r 2 -b 200000 -d Recurrent) & 0.40671 & \textbf{0.34814} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 5 -n 2 -v 2 -r 2 -b 200000 -d Recurrent) & 0.3309 & \textbf{0.00948} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 5 -n 5 -v 5 -r 2 -b 200000 -d Recurrent) & 0.46461 & \textbf{0.4605} \\
\bottomrule &  &  \\
\begin{tabularx}{\linewidth}{Xr}
		A \textbf{bold} value indicates higher accuracy, and \textit{\textbf{bold italics}} indicate a tie.  & \textbf{Unique Wins}
		\end{tabularx} & \textbf{0} & \textbf{32} \\
\cmidrule[0.4pt](lr){2-3} &  &  \\
\begin{tabularx}{\linewidth}{Xr} The test is a simple binomial test to determine whether the strategy in the rightmost 
             column is likely to have an equal number of ``wins'' as the strategy being compared against on the left. & \textbf{Test Statistics} \end{tabularx} & \textbf{p-value: 0} & \textbf{Confidence Interval:  0.91063 --- 1} \\


==> table105.tex <==
-s (RecurrentConceptDriftStream -x 200000 -y 200000 -z 100 -s (generators.AgrawalGenerator -f 2 -i 2) -d (generators.AgrawalGenerator -f 3 -i 3)) & 0.20846 & \textbf{0.17856} \\
-s (RecurrentConceptDriftStream -x 200000 -y 200000 -z 100 -s (generators.RandomTreeGenerator -r 1 -i 1) -d (generators.RandomTreeGenerator -r 2 -i 2)) & 0.22404 & \textbf{0.22004} \\
-s (RecurrentConceptDriftStream -x 200000 -y 200000 -z 100 -s (generators.SEAGenerator -f 2 -i 2) -d (generators.SEAGenerator -f 3 -i 3)) & 0.15251 & \textbf{0.14994} \\
-s (RecurrentConceptDriftStream -x 200000 -y 200000 -z 100 -s (generators.STAGGERGenerator -i 2 -f 2) -d (generators.STAGGERGenerator -i 3 -f 3)) & 0.1882 & \textbf{0.00435} \\
-s (generators.HyperplaneGenerator -k 10 -t 0.0001 -i 2) & 0.11566 & \textbf{0.11429} \\
-s (generators.HyperplaneGenerator -k 10 -t 0.001 -i 2) & 0.16785 & \textbf{0.16007} \\
-s (generators.HyperplaneGenerator -k 10 -t 0.01 -i 2) & 0.1713 & \textbf{0.1639} \\
-s (generators.HyperplaneGenerator -k 5 -t 0.0001 -i 2) & 0.1074 & \textbf{0.10719} \\
-s (generators.HyperplaneGenerator -k 5 -t 0.001 -i 2) & 0.16309 & \textbf{0.15347} \\
-s (generators.HyperplaneGenerator -k 5 -t 0.01 -i 2) & 0.17108 & \textbf{0.15901} \\
-s (generators.LEDGeneratorDrift -d 1 -i 2) & \textit{\textbf{0.26093}} & \textit{\textbf{0.26093}} \\
-s (generators.LEDGeneratorDrift -d 3 -i 2) & \textit{\textbf{0.26093}} & \textit{\textbf{0.26093}} \\
-s (generators.LEDGeneratorDrift -d 5 -i 2) & \textit{\textbf{0.26093}} & \textit{\textbf{0.26093}} \\
-s (generators.LEDGeneratorDrift -d 7 -i 2) & \textit{\textbf{0.26093}} & \textit{\textbf{0.26093}} \\
-s (generators.RandomRBFGeneratorDrift -s 0.0001 -k 10 -i 2 -r 2) & 0.11462 & \textbf{0.11451} \\
-s (generators.RandomRBFGeneratorDrift -s 0.0001 -k 50 -i 2 -r 2) & 0.2858 & \textbf{0.28429} \\
-s (generators.RandomRBFGeneratorDrift -s 0.001 -k 10 -i 2 -r 2) & \textbf{0.13821} & 0.13853 \\
-s (generators.RandomRBFGeneratorDrift -s 0.001 -k 50 -i 2 -r 2) & 0.40874 & \textbf{0.40525} \\
-s (generators.WaveformGeneratorDrift -d 1 -i 2 -n) & \textit{\textbf{0.16284}} & \textit{\textbf{0.16284}} \\
-s (generators.WaveformGeneratorDrift -d 3 -i 2 -n) & \textit{\textbf{0.16284}} & \textit{\textbf{0.16284}} \\
-s (generators.WaveformGeneratorDrift -d 5 -i 2 -n) & \textit{\textbf{0.16284}} & \textit{\textbf{0.16284}} \\
-s (generators.WaveformGeneratorDrift -d 7 -i 2 -n) & \textit{\textbf{0.16284}} & \textit{\textbf{0.16284}} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 2 -n 2 -v 2 -r 2 -b 200000 -d Recurrent) & 0.35403 & \textbf{0.00233} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 2 -v 2 -r 2 -b 200000 -d Recurrent) & 0.37862 & \textbf{0.00344} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 3 -v 2 -r 2 -b 200000 -d Recurrent) & 0.3504 & \textbf{0.01317} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 3 -v 3 -r 2 -b 200000 -d Recurrent) & 0.36505 & \textbf{0.05836} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 3 -v 4 -r 2 -b 200000 -d Recurrent) & 0.39687 & \textbf{0.15157} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 3 -v 5 -r 2 -b 200000 -d Recurrent) & 0.39622 & \textbf{0.23064} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 4 -n 2 -v 2 -r 2 -b 200000 -d Recurrent) & 0.33416 & \textbf{0.00933} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 4 -n 4 -v 4 -r 2 -b 200000 -d Recurrent) & 0.40671 & \textbf{0.34795} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 5 -n 2 -v 2 -r 2 -b 200000 -d Recurrent) & 0.3309 & \textbf{0.00972} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 5 -n 5 -v 5 -r 2 -b 200000 -d Recurrent) & 0.46461 & \textbf{0.46356} \\
\bottomrule &  &  \\
\begin{tabularx}{\linewidth}{Xr}
		A \textbf{bold} value indicates higher accuracy, and \textit{\textbf{bold italics}} indicate a tie.  & \textbf{Unique Wins}
		\end{tabularx} & \textbf{1} & \textbf{23} \\
\cmidrule[0.4pt](lr){2-3} &  &  \\
\begin{tabularx}{\linewidth}{Xr} The test is a simple binomial test to determine whether the strategy in the rightmost 
             column is likely to have an equal number of ``wins'' as the strategy being compared against on the left. & \textbf{Test Statistics} \end{tabularx} & \textbf{p-value: 0} & \textbf{Confidence Interval:  0.81711 --- 1} \\


==> table11.tex <==
-s (RecurrentConceptDriftStream -x 200000 -y 200000 -z 100 -s (generators.AgrawalGenerator -f 2 -i 2) -d (generators.AgrawalGenerator -f 3 -i 3)) & 0.13645 & \textbf{0.11303} \\
-s (RecurrentConceptDriftStream -x 200000 -y 200000 -z 100 -s (generators.RandomTreeGenerator -r 1 -i 1) -d (generators.RandomTreeGenerator -r 2 -i 2)) & 0.10104 & \textbf{0.09855} \\
-s (RecurrentConceptDriftStream -x 200000 -y 200000 -z 100 -s (generators.SEAGenerator -f 2 -i 2) -d (generators.SEAGenerator -f 3 -i 3)) & 0.12579 & \textbf{0.11203} \\
-s (RecurrentConceptDriftStream -x 200000 -y 200000 -z 100 -s (generators.STAGGERGenerator -i 2 -f 2) -d (generators.STAGGERGenerator -i 3 -f 3)) & 0.00215 & \textbf{0.00213} \\
-s (generators.HyperplaneGenerator -k 10 -t 0.0001 -i 2) & \textbf{0.10801} & 0.10882 \\
-s (generators.HyperplaneGenerator -k 10 -t 0.001 -i 2) & 0.11934 & \textbf{0.11838} \\
-s (generators.HyperplaneGenerator -k 10 -t 0.01 -i 2) & 0.1198 & \textbf{0.11943} \\
-s (generators.HyperplaneGenerator -k 5 -t 0.0001 -i 2) & \textbf{0.10588} & 0.10675 \\
-s (generators.HyperplaneGenerator -k 5 -t 0.001 -i 2) & 0.11254 & \textbf{0.11007} \\
-s (generators.HyperplaneGenerator -k 5 -t 0.01 -i 2) & 0.10767 & \textbf{0.10528} \\
-s (generators.LEDGeneratorDrift -d 1 -i 2) & 0.26137 & \textbf{0.26121} \\
-s (generators.LEDGeneratorDrift -d 3 -i 2) & 0.26137 & \textbf{0.26121} \\
-s (generators.LEDGeneratorDrift -d 5 -i 2) & 0.26137 & \textbf{0.26121} \\
-s (generators.LEDGeneratorDrift -d 7 -i 2) & 0.26137 & \textbf{0.26121} \\
-s (generators.RandomRBFGeneratorDrift -s 0.0001 -k 10 -i 2 -r 2) & 0.13508 & \textbf{0.11975} \\
-s (generators.RandomRBFGeneratorDrift -s 0.0001 -k 50 -i 2 -r 2) & 0.19549 & \textbf{0.19195} \\
-s (generators.RandomRBFGeneratorDrift -s 0.001 -k 10 -i 2 -r 2) & 0.16636 & \textbf{0.15236} \\
-s (generators.RandomRBFGeneratorDrift -s 0.001 -k 50 -i 2 -r 2) & 0.33926 & \textbf{0.33901} \\
-s (generators.WaveformGeneratorDrift -d 1 -i 2 -n) & \textbf{0.16279} & 0.16349 \\
-s (generators.WaveformGeneratorDrift -d 3 -i 2 -n) & \textbf{0.16279} & 0.16349 \\
-s (generators.WaveformGeneratorDrift -d 5 -i 2 -n) & \textbf{0.16279} & 0.16349 \\
-s (generators.WaveformGeneratorDrift -d 7 -i 2 -n) & \textbf{0.16279} & 0.16349 \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 2 -n 2 -v 2 -r 2 -b 200000 -d Recurrent) & 0.00185 & \textbf{0.00087} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 2 -v 2 -r 2 -b 200000 -d Recurrent) & 0.0016 & \textbf{0.00083} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 3 -v 2 -r 2 -b 200000 -d Recurrent) & 0.00252 & \textbf{0.00161} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 3 -v 3 -r 2 -b 200000 -d Recurrent) & 0.00425 & \textbf{0.00412} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 3 -v 4 -r 2 -b 200000 -d Recurrent) & 0.01212 & \textbf{0.01182} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 3 -v 5 -r 2 -b 200000 -d Recurrent) & 0.01687 & \textbf{0.0164} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 4 -n 2 -v 2 -r 2 -b 200000 -d Recurrent) & 0.00177 & \textbf{0.00101} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 4 -n 4 -v 4 -r 2 -b 200000 -d Recurrent) & 0.06662 & \textbf{0.06557} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 5 -n 2 -v 2 -r 2 -b 200000 -d Recurrent) & 0.00177 & \textbf{0.00104} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 5 -n 5 -v 5 -r 2 -b 200000 -d Recurrent) & 0.34892 & \textbf{0.34081} \\
\bottomrule &  &  \\
\begin{tabularx}{\linewidth}{Xr}
		A \textbf{bold} value indicates higher accuracy, and \textit{\textbf{bold italics}} indicate a tie.  & \textbf{Unique Wins}
		\end{tabularx} & \textbf{6} & \textbf{26} \\
\cmidrule[0.4pt](lr){2-3} &  &  \\
\begin{tabularx}{\linewidth}{Xr} The test is a simple binomial test to determine whether the strategy in the rightmost 
             column is likely to have an equal number of ``wins'' as the strategy being compared against on the left. & \textbf{Test Statistics} \end{tabularx} & \textbf{p-value: 0.00027} & \textbf{Confidence Interval:  0.66313 --- 1} \\


==> table12.tex <==
-s (RecurrentConceptDriftStream -x 200000 -y 200000 -z 100 -s (generators.AgrawalGenerator -f 2 -i 2) -d (generators.AgrawalGenerator -f 3 -i 3)) & 0.13645 & \textbf{0.12793} \\
-s (RecurrentConceptDriftStream -x 200000 -y 200000 -z 100 -s (generators.RandomTreeGenerator -r 1 -i 1) -d (generators.RandomTreeGenerator -r 2 -i 2)) & \textbf{0.10104} & 0.12227 \\
-s (RecurrentConceptDriftStream -x 200000 -y 200000 -z 100 -s (generators.SEAGenerator -f 2 -i 2) -d (generators.SEAGenerator -f 3 -i 3)) & 0.12579 & \textbf{0.11853} \\
-s (RecurrentConceptDriftStream -x 200000 -y 200000 -z 100 -s (generators.STAGGERGenerator -i 2 -f 2) -d (generators.STAGGERGenerator -i 3 -f 3)) & 0.00215 & \textbf{0.00188} \\
-s (generators.HyperplaneGenerator -k 10 -t 0.0001 -i 2) & \textbf{0.10801} & 0.11644 \\
-s (generators.HyperplaneGenerator -k 10 -t 0.001 -i 2) & \textbf{0.11934} & 0.1241 \\
-s (generators.HyperplaneGenerator -k 10 -t 0.01 -i 2) & \textbf{0.1198} & 0.12509 \\
-s (generators.HyperplaneGenerator -k 5 -t 0.0001 -i 2) & \textbf{0.10588} & 0.11753 \\
-s (generators.HyperplaneGenerator -k 5 -t 0.001 -i 2) & \textbf{0.11254} & 0.11526 \\
-s (generators.HyperplaneGenerator -k 5 -t 0.01 -i 2) & \textbf{0.10767} & 0.10867 \\
-s (generators.LEDGeneratorDrift -d 1 -i 2) & 0.26137 & \textbf{0.26124} \\
-s (generators.LEDGeneratorDrift -d 3 -i 2) & 0.26137 & \textbf{0.26124} \\
-s (generators.LEDGeneratorDrift -d 5 -i 2) & 0.26137 & \textbf{0.26124} \\
-s (generators.LEDGeneratorDrift -d 7 -i 2) & 0.26137 & \textbf{0.26124} \\
-s (generators.RandomRBFGeneratorDrift -s 0.0001 -k 10 -i 2 -r 2) & 0.13508 & \textbf{0.12037} \\
-s (generators.RandomRBFGeneratorDrift -s 0.0001 -k 50 -i 2 -r 2) & 0.19549 & \textbf{0.18017} \\
-s (generators.RandomRBFGeneratorDrift -s 0.001 -k 10 -i 2 -r 2) & 0.16636 & \textbf{0.15522} \\
-s (generators.RandomRBFGeneratorDrift -s 0.001 -k 50 -i 2 -r 2) & 0.33926 & \textbf{0.32757} \\
-s (generators.WaveformGeneratorDrift -d 1 -i 2 -n) & \textbf{0.16279} & 0.17118 \\
-s (generators.WaveformGeneratorDrift -d 3 -i 2 -n) & \textbf{0.16279} & 0.17118 \\
-s (generators.WaveformGeneratorDrift -d 5 -i 2 -n) & \textbf{0.16279} & 0.17118 \\
-s (generators.WaveformGeneratorDrift -d 7 -i 2 -n) & \textbf{0.16279} & 0.17118 \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 2 -n 2 -v 2 -r 2 -b 200000 -d Recurrent) & 0.00185 & \textbf{0.00068} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 2 -v 2 -r 2 -b 200000 -d Recurrent) & 0.0016 & \textbf{0.00062} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 3 -v 2 -r 2 -b 200000 -d Recurrent) & 0.00252 & \textbf{0.00122} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 3 -v 3 -r 2 -b 200000 -d Recurrent) & 0.00425 & \textbf{0.00307} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 3 -v 4 -r 2 -b 200000 -d Recurrent) & 0.01212 & \textbf{0.0093} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 3 -v 5 -r 2 -b 200000 -d Recurrent) & 0.01687 & \textbf{0.01475} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 4 -n 2 -v 2 -r 2 -b 200000 -d Recurrent) & 0.00177 & \textbf{0.00073} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 4 -n 4 -v 4 -r 2 -b 200000 -d Recurrent) & 0.06662 & \textbf{0.05314} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 5 -n 2 -v 2 -r 2 -b 200000 -d Recurrent) & 0.00177 & \textbf{0.00078} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 5 -n 5 -v 5 -r 2 -b 200000 -d Recurrent) & 0.34892 & \textbf{0.28637} \\
\bottomrule &  &  \\
\begin{tabularx}{\linewidth}{Xr}
		A \textbf{bold} value indicates higher accuracy, and \textit{\textbf{bold italics}} indicate a tie.  & \textbf{Unique Wins}
		\end{tabularx} & \textbf{11} & \textbf{21} \\
\cmidrule[0.4pt](lr){2-3} &  &  \\
\begin{tabularx}{\linewidth}{Xr} The test is a simple binomial test to determine whether the strategy in the rightmost 
             column is likely to have an equal number of ``wins'' as the strategy being compared against on the left. & \textbf{Test Statistics} \end{tabularx} & \textbf{p-value: 0.05509} & \textbf{Confidence Interval:  0.49581 --- 1} \\


==> table2.tex <==
-s (RecurrentConceptDriftStream -x 200000 -y 200000 -z 100 -s (generators.AgrawalGenerator -f 2 -i 2) -d (generators.AgrawalGenerator -f 3 -i 3)) & \textit{\textbf{0.13643}} & \textit{\textbf{0.13643}} \\
-s (RecurrentConceptDriftStream -x 200000 -y 200000 -z 100 -s (generators.RandomTreeGenerator -r 1 -i 1) -d (generators.RandomTreeGenerator -r 2 -i 2)) & 0.10663 & \textbf{0.10615} \\
-s (RecurrentConceptDriftStream -x 200000 -y 200000 -z 100 -s (generators.SEAGenerator -f 2 -i 2) -d (generators.SEAGenerator -f 3 -i 3)) & \textit{\textbf{0.12538}} & \textit{\textbf{0.12538}} \\
-s (RecurrentConceptDriftStream -x 200000 -y 200000 -z 100 -s (generators.STAGGERGenerator -i 2 -f 2) -d (generators.STAGGERGenerator -i 3 -f 3)) & \textit{\textbf{0.00136}} & \textit{\textbf{0.00136}} \\
-s (generators.HyperplaneGenerator -k 10 -t 0.0001 -i 2) & \textbf{0.10562} & 0.10576 \\
-s (generators.HyperplaneGenerator -k 10 -t 0.001 -i 2) & \textbf{0.11571} & 0.11606 \\
-s (generators.HyperplaneGenerator -k 10 -t 0.01 -i 2) & 0.11705 & \textbf{0.11681} \\
-s (generators.HyperplaneGenerator -k 5 -t 0.0001 -i 2) & 0.1044 & \textbf{0.10412} \\
-s (generators.HyperplaneGenerator -k 5 -t 0.001 -i 2) & 0.10963 & \textbf{0.10947} \\
-s (generators.HyperplaneGenerator -k 5 -t 0.01 -i 2) & \textbf{0.10469} & 0.1047 \\
-s (generators.LEDGeneratorDrift -d 1 -i 2) & 0.26127 & \textbf{0.26123} \\
-s (generators.LEDGeneratorDrift -d 3 -i 2) & 0.26127 & \textbf{0.26123} \\
-s (generators.LEDGeneratorDrift -d 5 -i 2) & 0.26127 & \textbf{0.26123} \\
-s (generators.LEDGeneratorDrift -d 7 -i 2) & 0.26127 & \textbf{0.26123} \\
-s (generators.RandomRBFGeneratorDrift -s 0.0001 -k 10 -i 2 -r 2) & 0.13617 & \textbf{0.13109} \\
-s (generators.RandomRBFGeneratorDrift -s 0.0001 -k 50 -i 2 -r 2) & 0.18238 & \textbf{0.18094} \\
-s (generators.RandomRBFGeneratorDrift -s 0.001 -k 10 -i 2 -r 2) & 0.17105 & \textbf{0.16503} \\
-s (generators.RandomRBFGeneratorDrift -s 0.001 -k 50 -i 2 -r 2) & \textbf{0.32534} & 0.32535 \\
-s (generators.WaveformGeneratorDrift -d 1 -i 2 -n) & \textbf{0.16234} & 0.16251 \\
-s (generators.WaveformGeneratorDrift -d 3 -i 2 -n) & \textbf{0.16234} & 0.16251 \\
-s (generators.WaveformGeneratorDrift -d 5 -i 2 -n) & \textbf{0.16234} & 0.16251 \\
-s (generators.WaveformGeneratorDrift -d 7 -i 2 -n) & \textbf{0.16234} & 0.16251 \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 2 -n 2 -v 2 -r 2 -b 200000 -d Recurrent) & \textit{\textbf{7e-04}} & \textit{\textbf{7e-04}} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 2 -v 2 -r 2 -b 200000 -d Recurrent) & \textit{\textbf{0.00056}} & \textit{\textbf{0.00056}} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 3 -v 2 -r 2 -b 200000 -d Recurrent) & 0.00157 & \textbf{0.00144} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 3 -v 3 -r 2 -b 200000 -d Recurrent) & 0.00793 & \textbf{0.00475} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 3 -v 4 -r 2 -b 200000 -d Recurrent) & 0.01693 & \textbf{0.01389} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 3 -v 5 -r 2 -b 200000 -d Recurrent) & 0.0212 & \textbf{0.01978} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 4 -n 2 -v 2 -r 2 -b 200000 -d Recurrent) & \textit{\textbf{0.00049}} & \textit{\textbf{0.00049}} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 4 -n 4 -v 4 -r 2 -b 200000 -d Recurrent) & 0.07469 & \textbf{0.07347} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 5 -n 2 -v 2 -r 2 -b 200000 -d Recurrent) & \textit{\textbf{0.00037}} & \textit{\textbf{0.00037}} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 5 -n 5 -v 5 -r 2 -b 200000 -d Recurrent) & 0.35638 & \textbf{0.35605} \\
\bottomrule &  &  \\
\begin{tabularx}{\linewidth}{Xr}
		A \textbf{bold} value indicates higher accuracy, and \textit{\textbf{bold italics}} indicate a tie.  & \textbf{Unique Wins}
		\end{tabularx} & \textbf{8} & \textbf{17} \\
\cmidrule[0.4pt](lr){2-3} &  &  \\
\begin{tabularx}{\linewidth}{Xr} The test is a simple binomial test to determine whether the strategy in the rightmost 
             column is likely to have an equal number of ``wins'' as the strategy being compared against on the left. & \textbf{Test Statistics} \end{tabularx} & \textbf{p-value: 0.05388} & \textbf{Confidence Interval:  0.49636 --- 1} \\


==> table3.tex <==
-s (RecurrentConceptDriftStream -x 200000 -y 200000 -z 100 -s (generators.AgrawalGenerator -f 2 -i 2) -d (generators.AgrawalGenerator -f 3 -i 3)) & \textbf{0.1364} & 0.13643 \\
-s (RecurrentConceptDriftStream -x 200000 -y 200000 -z 100 -s (generators.RandomTreeGenerator -r 1 -i 1) -d (generators.RandomTreeGenerator -r 2 -i 2)) & \textbf{0.10284} & 0.10663 \\
-s (RecurrentConceptDriftStream -x 200000 -y 200000 -z 100 -s (generators.SEAGenerator -f 2 -i 2) -d (generators.SEAGenerator -f 3 -i 3)) & 0.1256 & \textbf{0.12538} \\
-s (RecurrentConceptDriftStream -x 200000 -y 200000 -z 100 -s (generators.STAGGERGenerator -i 2 -f 2) -d (generators.STAGGERGenerator -i 3 -f 3)) & 0.002 & \textbf{0.00136} \\
-s (generators.HyperplaneGenerator -k 10 -t 0.0001 -i 2) & 0.13141 & \textbf{0.10562} \\
-s (generators.HyperplaneGenerator -k 10 -t 0.001 -i 2) & 0.12012 & \textbf{0.11571} \\
-s (generators.HyperplaneGenerator -k 10 -t 0.01 -i 2) & 0.12594 & \textbf{0.11705} \\
-s (generators.HyperplaneGenerator -k 5 -t 0.0001 -i 2) & 0.13913 & \textbf{0.1044} \\
-s (generators.HyperplaneGenerator -k 5 -t 0.001 -i 2) & 0.11189 & \textbf{0.10963} \\
-s (generators.HyperplaneGenerator -k 5 -t 0.01 -i 2) & 0.10566 & \textbf{0.10469} \\
-s (generators.LEDGeneratorDrift -d 1 -i 2) & 0.26138 & \textbf{0.26127} \\
-s (generators.LEDGeneratorDrift -d 3 -i 2) & 0.26138 & \textbf{0.26127} \\
-s (generators.LEDGeneratorDrift -d 5 -i 2) & 0.26138 & \textbf{0.26127} \\
-s (generators.LEDGeneratorDrift -d 7 -i 2) & 0.26138 & \textbf{0.26127} \\
-s (generators.RandomRBFGeneratorDrift -s 0.0001 -k 10 -i 2 -r 2) & 0.14943 & \textbf{0.13617} \\
-s (generators.RandomRBFGeneratorDrift -s 0.0001 -k 50 -i 2 -r 2) & 0.19643 & \textbf{0.18238} \\
-s (generators.RandomRBFGeneratorDrift -s 0.001 -k 10 -i 2 -r 2) & 0.20134 & \textbf{0.17105} \\
-s (generators.RandomRBFGeneratorDrift -s 0.001 -k 50 -i 2 -r 2) & 0.33891 & \textbf{0.32534} \\
-s (generators.WaveformGeneratorDrift -d 1 -i 2 -n) & 0.16866 & \textbf{0.16234} \\
-s (generators.WaveformGeneratorDrift -d 3 -i 2 -n) & 0.16866 & \textbf{0.16234} \\
-s (generators.WaveformGeneratorDrift -d 5 -i 2 -n) & 0.16866 & \textbf{0.16234} \\
-s (generators.WaveformGeneratorDrift -d 7 -i 2 -n) & 0.16866 & \textbf{0.16234} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 2 -n 2 -v 2 -r 2 -b 200000 -d Recurrent) & 0.00159 & \textbf{7e-04} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 2 -v 2 -r 2 -b 200000 -d Recurrent) & 0.00147 & \textbf{0.00056} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 3 -v 2 -r 2 -b 200000 -d Recurrent) & 0.00246 & \textbf{0.00157} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 3 -v 3 -r 2 -b 200000 -d Recurrent) & \textbf{0.00699} & 0.00793 \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 3 -v 4 -r 2 -b 200000 -d Recurrent) & \textbf{0.01497} & 0.01693 \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 3 -v 5 -r 2 -b 200000 -d Recurrent) & \textbf{0.01796} & 0.0212 \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 4 -n 2 -v 2 -r 2 -b 200000 -d Recurrent) & 0.00149 & \textbf{0.00049} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 4 -n 4 -v 4 -r 2 -b 200000 -d Recurrent) & \textbf{0.06767} & 0.07469 \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 5 -n 2 -v 2 -r 2 -b 200000 -d Recurrent) & 0.00148 & \textbf{0.00037} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 5 -n 5 -v 5 -r 2 -b 200000 -d Recurrent) & \textbf{0.34955} & 0.35638 \\
\bottomrule &  &  \\
\begin{tabularx}{\linewidth}{Xr}
		A \textbf{bold} value indicates higher accuracy, and \textit{\textbf{bold italics}} indicate a tie.  & \textbf{Unique Wins}
		\end{tabularx} & \textbf{7} & \textbf{25} \\
\cmidrule[0.4pt](lr){2-3} &  &  \\
\begin{tabularx}{\linewidth}{Xr} The test is a simple binomial test to determine whether the strategy in the rightmost 
             column is likely to have an equal number of ``wins'' as the strategy being compared against on the left. & \textbf{Test Statistics} \end{tabularx} & \textbf{p-value: 0.00105} & \textbf{Confidence Interval:  0.6281 --- 1} \\


==> table4.tex <==
-s (RecurrentConceptDriftStream -x 200000 -y 200000 -z 100 -s (generators.AgrawalGenerator -f 2 -i 2) -d (generators.AgrawalGenerator -f 3 -i 3)) & 0.1364 & \textbf{0.13354} \\
-s (RecurrentConceptDriftStream -x 200000 -y 200000 -z 100 -s (generators.RandomTreeGenerator -r 1 -i 1) -d (generators.RandomTreeGenerator -r 2 -i 2)) & 0.10284 & \textbf{0.10111} \\
-s (RecurrentConceptDriftStream -x 200000 -y 200000 -z 100 -s (generators.SEAGenerator -f 2 -i 2) -d (generators.SEAGenerator -f 3 -i 3)) & 0.1256 & \textbf{0.12522} \\
-s (RecurrentConceptDriftStream -x 200000 -y 200000 -z 100 -s (generators.STAGGERGenerator -i 2 -f 2) -d (generators.STAGGERGenerator -i 3 -f 3)) & \textbf{0.002} & 0.00205 \\
-s (generators.HyperplaneGenerator -k 10 -t 0.0001 -i 2) & \textbf{0.13141} & 0.15097 \\
-s (generators.HyperplaneGenerator -k 10 -t 0.001 -i 2) & \textbf{0.12012} & 0.14423 \\
-s (generators.HyperplaneGenerator -k 10 -t 0.01 -i 2) & 0.12594 & \textbf{0.12496} \\
-s (generators.HyperplaneGenerator -k 5 -t 0.0001 -i 2) & 0.13913 & \textbf{0.13817} \\
-s (generators.HyperplaneGenerator -k 5 -t 0.001 -i 2) & \textbf{0.11189} & 0.11276 \\
-s (generators.HyperplaneGenerator -k 5 -t 0.01 -i 2) & \textbf{0.10566} & 0.10773 \\
-s (generators.LEDGeneratorDrift -d 1 -i 2) & 0.26138 & \textbf{0.26114} \\
-s (generators.LEDGeneratorDrift -d 3 -i 2) & 0.26138 & \textbf{0.26114} \\
-s (generators.LEDGeneratorDrift -d 5 -i 2) & 0.26138 & \textbf{0.26114} \\
-s (generators.LEDGeneratorDrift -d 7 -i 2) & 0.26138 & \textbf{0.26114} \\
-s (generators.RandomRBFGeneratorDrift -s 0.0001 -k 10 -i 2 -r 2) & 0.14943 & \textbf{0.1475} \\
-s (generators.RandomRBFGeneratorDrift -s 0.0001 -k 50 -i 2 -r 2) & 0.19643 & \textbf{0.18406} \\
-s (generators.RandomRBFGeneratorDrift -s 0.001 -k 10 -i 2 -r 2) & 0.20134 & \textbf{0.19871} \\
-s (generators.RandomRBFGeneratorDrift -s 0.001 -k 50 -i 2 -r 2) & 0.33891 & \textbf{0.32724} \\
-s (generators.WaveformGeneratorDrift -d 1 -i 2 -n) & \textbf{0.16866} & 0.1749 \\
-s (generators.WaveformGeneratorDrift -d 3 -i 2 -n) & \textbf{0.16866} & 0.1749 \\
-s (generators.WaveformGeneratorDrift -d 5 -i 2 -n) & \textbf{0.16866} & 0.1749 \\
-s (generators.WaveformGeneratorDrift -d 7 -i 2 -n) & \textbf{0.16866} & 0.1749 \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 2 -n 2 -v 2 -r 2 -b 200000 -d Recurrent) & 0.00159 & \textbf{0.00154} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 2 -v 2 -r 2 -b 200000 -d Recurrent) & 0.00147 & \textbf{0.00135} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 3 -v 2 -r 2 -b 200000 -d Recurrent) & 0.00246 & \textbf{0.00185} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 3 -v 3 -r 2 -b 200000 -d Recurrent) & 0.00699 & \textbf{0.00698} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 3 -v 4 -r 2 -b 200000 -d Recurrent) & 0.01497 & \textbf{0.01312} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 3 -v 5 -r 2 -b 200000 -d Recurrent) & 0.01796 & \textbf{0.01528} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 4 -n 2 -v 2 -r 2 -b 200000 -d Recurrent) & 0.00149 & \textbf{0.00146} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 4 -n 4 -v 4 -r 2 -b 200000 -d Recurrent) & 0.06767 & \textbf{0.05249} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 5 -n 2 -v 2 -r 2 -b 200000 -d Recurrent) & 0.00148 & \textbf{0.00143} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 5 -n 5 -v 5 -r 2 -b 200000 -d Recurrent) & 0.34955 & \textbf{0.28932} \\
\bottomrule &  &  \\
\begin{tabularx}{\linewidth}{Xr}
		A \textbf{bold} value indicates higher accuracy, and \textit{\textbf{bold italics}} indicate a tie.  & \textbf{Unique Wins}
		\end{tabularx} & \textbf{9} & \textbf{23} \\
\cmidrule[0.4pt](lr){2-3} &  &  \\
\begin{tabularx}{\linewidth}{Xr} The test is a simple binomial test to determine whether the strategy in the rightmost 
             column is likely to have an equal number of ``wins'' as the strategy being compared against on the left. & \textbf{Test Statistics} \end{tabularx} & \textbf{p-value: 0.01003} & \textbf{Confidence Interval:  0.56055 --- 1} \\


==> table5.tex <==
-s (RecurrentConceptDriftStream -x 200000 -y 200000 -z 100 -s (generators.AgrawalGenerator -f 2 -i 2) -d (generators.AgrawalGenerator -f 3 -i 3)) & \textit{\textbf{0.13645}} & \textit{\textbf{0.13645}} \\
-s (RecurrentConceptDriftStream -x 200000 -y 200000 -z 100 -s (generators.RandomTreeGenerator -r 1 -i 1) -d (generators.RandomTreeGenerator -r 2 -i 2)) & \textit{\textbf{0.10104}} & \textit{\textbf{0.10104}} \\
-s (RecurrentConceptDriftStream -x 200000 -y 200000 -z 100 -s (generators.SEAGenerator -f 2 -i 2) -d (generators.SEAGenerator -f 3 -i 3)) & \textit{\textbf{0.12579}} & \textit{\textbf{0.12579}} \\
-s (RecurrentConceptDriftStream -x 200000 -y 200000 -z 100 -s (generators.STAGGERGenerator -i 2 -f 2) -d (generators.STAGGERGenerator -i 3 -f 3)) & \textit{\textbf{0.00215}} & \textit{\textbf{0.00215}} \\
-s (generators.HyperplaneGenerator -k 10 -t 0.0001 -i 2) & \textit{\textbf{0.10801}} & \textit{\textbf{0.10801}} \\
-s (generators.HyperplaneGenerator -k 10 -t 0.001 -i 2) & \textit{\textbf{0.11934}} & \textit{\textbf{0.11934}} \\
-s (generators.HyperplaneGenerator -k 10 -t 0.01 -i 2) & \textit{\textbf{0.1198}} & \textit{\textbf{0.1198}} \\
-s (generators.HyperplaneGenerator -k 5 -t 0.0001 -i 2) & \textit{\textbf{0.10588}} & \textit{\textbf{0.10588}} \\
-s (generators.HyperplaneGenerator -k 5 -t 0.001 -i 2) & \textit{\textbf{0.11254}} & \textit{\textbf{0.11254}} \\
-s (generators.HyperplaneGenerator -k 5 -t 0.01 -i 2) & \textit{\textbf{0.10767}} & \textit{\textbf{0.10767}} \\
-s (generators.LEDGeneratorDrift -d 1 -i 2) & \textit{\textbf{0.26137}} & \textit{\textbf{0.26137}} \\
-s (generators.LEDGeneratorDrift -d 3 -i 2) & \textit{\textbf{0.26137}} & \textit{\textbf{0.26137}} \\
-s (generators.LEDGeneratorDrift -d 5 -i 2) & \textit{\textbf{0.26137}} & \textit{\textbf{0.26137}} \\
-s (generators.LEDGeneratorDrift -d 7 -i 2) & \textit{\textbf{0.26137}} & \textit{\textbf{0.26137}} \\
-s (generators.RandomRBFGeneratorDrift -s 0.0001 -k 10 -i 2 -r 2) & \textit{\textbf{0.13508}} & \textit{\textbf{0.13508}} \\
-s (generators.RandomRBFGeneratorDrift -s 0.0001 -k 50 -i 2 -r 2) & \textit{\textbf{0.19549}} & \textit{\textbf{0.19549}} \\
-s (generators.RandomRBFGeneratorDrift -s 0.001 -k 10 -i 2 -r 2) & \textit{\textbf{0.16636}} & \textit{\textbf{0.16636}} \\
-s (generators.RandomRBFGeneratorDrift -s 0.001 -k 50 -i 2 -r 2) & \textit{\textbf{0.33926}} & \textit{\textbf{0.33926}} \\
-s (generators.WaveformGeneratorDrift -d 1 -i 2 -n) & \textit{\textbf{0.16279}} & \textit{\textbf{0.16279}} \\
-s (generators.WaveformGeneratorDrift -d 3 -i 2 -n) & \textit{\textbf{0.16279}} & \textit{\textbf{0.16279}} \\
-s (generators.WaveformGeneratorDrift -d 5 -i 2 -n) & \textit{\textbf{0.16279}} & \textit{\textbf{0.16279}} \\
-s (generators.WaveformGeneratorDrift -d 7 -i 2 -n) & \textit{\textbf{0.16279}} & \textit{\textbf{0.16279}} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 2 -n 2 -v 2 -r 2 -b 200000 -d Recurrent) & \textit{\textbf{0.00185}} & \textit{\textbf{0.00185}} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 2 -v 2 -r 2 -b 200000 -d Recurrent) & \textit{\textbf{0.0016}} & \textit{\textbf{0.0016}} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 3 -v 2 -r 2 -b 200000 -d Recurrent) & \textit{\textbf{0.00252}} & \textit{\textbf{0.00252}} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 3 -v 3 -r 2 -b 200000 -d Recurrent) & \textit{\textbf{0.00425}} & \textit{\textbf{0.00425}} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 3 -v 4 -r 2 -b 200000 -d Recurrent) & \textit{\textbf{0.01212}} & \textit{\textbf{0.01212}} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 3 -v 5 -r 2 -b 200000 -d Recurrent) & \textit{\textbf{0.01687}} & \textit{\textbf{0.01687}} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 4 -n 2 -v 2 -r 2 -b 200000 -d Recurrent) & \textit{\textbf{0.00177}} & \textit{\textbf{0.00177}} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 4 -n 4 -v 4 -r 2 -b 200000 -d Recurrent) & \textit{\textbf{0.06662}} & \textit{\textbf{0.06662}} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 5 -n 2 -v 2 -r 2 -b 200000 -d Recurrent) & \textit{\textbf{0.00177}} & \textit{\textbf{0.00177}} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 5 -n 5 -v 5 -r 2 -b 200000 -d Recurrent) & \textit{\textbf{0.34892}} & \textit{\textbf{0.34892}} \\


==> table6.tex <==
-s (RecurrentConceptDriftStream -x 200000 -y 200000 -z 100 -s (generators.AgrawalGenerator -f 2 -i 2) -d (generators.AgrawalGenerator -f 3 -i 3)) & 0.13645 & \textbf{0.12454} \\
-s (RecurrentConceptDriftStream -x 200000 -y 200000 -z 100 -s (generators.RandomTreeGenerator -r 1 -i 1) -d (generators.RandomTreeGenerator -r 2 -i 2)) & 0.10104 & \textbf{0.09866} \\
-s (RecurrentConceptDriftStream -x 200000 -y 200000 -z 100 -s (generators.SEAGenerator -f 2 -i 2) -d (generators.SEAGenerator -f 3 -i 3)) & 0.12579 & \textbf{0.11207} \\
-s (RecurrentConceptDriftStream -x 200000 -y 200000 -z 100 -s (generators.STAGGERGenerator -i 2 -f 2) -d (generators.STAGGERGenerator -i 3 -f 3)) & 0.00215 & \textbf{0.00213} \\
-s (generators.HyperplaneGenerator -k 10 -t 0.0001 -i 2) & \textbf{0.10801} & 0.10875 \\
-s (generators.HyperplaneGenerator -k 10 -t 0.001 -i 2) & 0.11934 & \textbf{0.11823} \\
-s (generators.HyperplaneGenerator -k 10 -t 0.01 -i 2) & 0.1198 & \textbf{0.11948} \\
-s (generators.HyperplaneGenerator -k 5 -t 0.0001 -i 2) & \textbf{0.10588} & 0.10693 \\
-s (generators.HyperplaneGenerator -k 5 -t 0.001 -i 2) & 0.11254 & \textbf{0.11008} \\
-s (generators.HyperplaneGenerator -k 5 -t 0.01 -i 2) & 0.10767 & \textbf{0.1049} \\
-s (generators.LEDGeneratorDrift -d 1 -i 2) & \textit{\textbf{0.26137}} & \textit{\textbf{0.26137}} \\
-s (generators.LEDGeneratorDrift -d 3 -i 2) & \textit{\textbf{0.26137}} & \textit{\textbf{0.26137}} \\
-s (generators.LEDGeneratorDrift -d 5 -i 2) & \textit{\textbf{0.26137}} & \textit{\textbf{0.26137}} \\
-s (generators.LEDGeneratorDrift -d 7 -i 2) & \textit{\textbf{0.26137}} & \textit{\textbf{0.26137}} \\
-s (generators.RandomRBFGeneratorDrift -s 0.0001 -k 10 -i 2 -r 2) & 0.13508 & \textbf{0.1197} \\
-s (generators.RandomRBFGeneratorDrift -s 0.0001 -k 50 -i 2 -r 2) & 0.19549 & \textbf{0.19199} \\
-s (generators.RandomRBFGeneratorDrift -s 0.001 -k 10 -i 2 -r 2) & 0.16636 & \textbf{0.15267} \\
-s (generators.RandomRBFGeneratorDrift -s 0.001 -k 50 -i 2 -r 2) & 0.33926 & \textbf{0.33877} \\
-s (generators.WaveformGeneratorDrift -d 1 -i 2 -n) & \textbf{0.16279} & 0.16337 \\
-s (generators.WaveformGeneratorDrift -d 3 -i 2 -n) & \textbf{0.16279} & 0.16337 \\
-s (generators.WaveformGeneratorDrift -d 5 -i 2 -n) & \textbf{0.16279} & 0.16337 \\
-s (generators.WaveformGeneratorDrift -d 7 -i 2 -n) & \textbf{0.16279} & 0.16337 \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 2 -n 2 -v 2 -r 2 -b 200000 -d Recurrent) & 0.00185 & \textbf{0.00085} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 2 -v 2 -r 2 -b 200000 -d Recurrent) & 0.0016 & \textbf{0.00087} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 3 -v 2 -r 2 -b 200000 -d Recurrent) & 0.00252 & \textbf{0.00169} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 3 -v 3 -r 2 -b 200000 -d Recurrent) & 0.00425 & \textbf{0.00404} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 3 -v 4 -r 2 -b 200000 -d Recurrent) & \textbf{0.01212} & 0.01228 \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 3 -v 5 -r 2 -b 200000 -d Recurrent) & 0.01687 & \textbf{0.01675} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 4 -n 2 -v 2 -r 2 -b 200000 -d Recurrent) & 0.00177 & \textbf{0.00095} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 4 -n 4 -v 4 -r 2 -b 200000 -d Recurrent) & 0.06662 & \textbf{0.06643} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 5 -n 2 -v 2 -r 2 -b 200000 -d Recurrent) & 0.00177 & \textbf{0.00113} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 5 -n 5 -v 5 -r 2 -b 200000 -d Recurrent) & \textit{\textbf{0.34892}} & \textit{\textbf{0.34892}} \\
\bottomrule &  &  \\
\begin{tabularx}{\linewidth}{Xr}
		A \textbf{bold} value indicates higher accuracy, and \textit{\textbf{bold italics}} indicate a tie.  & \textbf{Unique Wins}
		\end{tabularx} & \textbf{7} & \textbf{20} \\
\cmidrule[0.4pt](lr){2-3} &  &  \\
\begin{tabularx}{\linewidth}{Xr} The test is a simple binomial test to determine whether the strategy in the rightmost 
             column is likely to have an equal number of ``wins'' as the strategy being compared against on the left. & \textbf{Test Statistics} \end{tabularx} & \textbf{p-value: 0.00958} & \textbf{Confidence Interval:  0.5677 --- 1} \\


==> table7.tex <==
-s (RecurrentConceptDriftStream -x 200000 -y 200000 -z 100 -s (generators.AgrawalGenerator -f 2 -i 2) -d (generators.AgrawalGenerator -f 3 -i 3)) & \textbf{0.13645} & 0.13871 \\
-s (RecurrentConceptDriftStream -x 200000 -y 200000 -z 100 -s (generators.RandomTreeGenerator -r 1 -i 1) -d (generators.RandomTreeGenerator -r 2 -i 2)) & 0.10104 & \textbf{0.10079} \\
-s (RecurrentConceptDriftStream -x 200000 -y 200000 -z 100 -s (generators.SEAGenerator -f 2 -i 2) -d (generators.SEAGenerator -f 3 -i 3)) & 0.12579 & \textbf{0.12578} \\
-s (RecurrentConceptDriftStream -x 200000 -y 200000 -z 100 -s (generators.STAGGERGenerator -i 2 -f 2) -d (generators.STAGGERGenerator -i 3 -f 3)) & \textit{\textbf{0.00215}} & \textit{\textbf{0.00215}} \\
-s (generators.HyperplaneGenerator -k 10 -t 0.0001 -i 2) & \textbf{0.10801} & 0.10832 \\
-s (generators.HyperplaneGenerator -k 10 -t 0.001 -i 2) & 0.11934 & \textbf{0.11929} \\
-s (generators.HyperplaneGenerator -k 10 -t 0.01 -i 2) & 0.1198 & \textbf{0.11979} \\
-s (generators.HyperplaneGenerator -k 5 -t 0.0001 -i 2) & \textbf{0.10588} & 0.1063 \\
-s (generators.HyperplaneGenerator -k 5 -t 0.001 -i 2) & 0.11254 & \textbf{0.11148} \\
-s (generators.HyperplaneGenerator -k 5 -t 0.01 -i 2) & \textbf{0.10767} & 0.1083 \\
-s (generators.LEDGeneratorDrift -d 1 -i 2) & 0.26137 & \textbf{0.26121} \\
-s (generators.LEDGeneratorDrift -d 3 -i 2) & 0.26137 & \textbf{0.26121} \\
-s (generators.LEDGeneratorDrift -d 5 -i 2) & 0.26137 & \textbf{0.26121} \\
-s (generators.LEDGeneratorDrift -d 7 -i 2) & 0.26137 & \textbf{0.26121} \\
-s (generators.RandomRBFGeneratorDrift -s 0.0001 -k 10 -i 2 -r 2) & \textbf{0.13508} & 0.1372 \\
-s (generators.RandomRBFGeneratorDrift -s 0.0001 -k 50 -i 2 -r 2) & 0.19549 & \textbf{0.19518} \\
-s (generators.RandomRBFGeneratorDrift -s 0.001 -k 10 -i 2 -r 2) & 0.16636 & \textbf{0.16541} \\
-s (generators.RandomRBFGeneratorDrift -s 0.001 -k 50 -i 2 -r 2) & \textbf{0.33926} & 0.33939 \\
-s (generators.WaveformGeneratorDrift -d 1 -i 2 -n) & 0.16279 & \textbf{0.1625} \\
-s (generators.WaveformGeneratorDrift -d 3 -i 2 -n) & 0.16279 & \textbf{0.1625} \\
-s (generators.WaveformGeneratorDrift -d 5 -i 2 -n) & 0.16279 & \textbf{0.1625} \\
-s (generators.WaveformGeneratorDrift -d 7 -i 2 -n) & 0.16279 & \textbf{0.1625} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 2 -n 2 -v 2 -r 2 -b 200000 -d Recurrent) & 0.00185 & \textbf{0.00183} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 2 -v 2 -r 2 -b 200000 -d Recurrent) & \textbf{0.0016} & 0.00161 \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 3 -v 2 -r 2 -b 200000 -d Recurrent) & \textbf{0.00252} & 0.0028 \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 3 -v 3 -r 2 -b 200000 -d Recurrent) & 0.00425 & \textbf{0.00421} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 3 -v 4 -r 2 -b 200000 -d Recurrent) & 0.01212 & \textbf{0.0118} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 3 -v 5 -r 2 -b 200000 -d Recurrent) & 0.01687 & \textbf{0.01646} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 4 -n 2 -v 2 -r 2 -b 200000 -d Recurrent) & 0.00177 & \textbf{0.00176} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 4 -n 4 -v 4 -r 2 -b 200000 -d Recurrent) & 0.06662 & \textbf{0.06559} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 5 -n 2 -v 2 -r 2 -b 200000 -d Recurrent) & 0.00177 & \textbf{0.00173} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 5 -n 5 -v 5 -r 2 -b 200000 -d Recurrent) & 0.34892 & \textbf{0.34081} \\
\bottomrule &  &  \\
\begin{tabularx}{\linewidth}{Xr}
		A \textbf{bold} value indicates higher accuracy, and \textit{\textbf{bold italics}} indicate a tie.  & \textbf{Unique Wins}
		\end{tabularx} & \textbf{8} & \textbf{23} \\
\cmidrule[0.4pt](lr){2-3} &  &  \\
\begin{tabularx}{\linewidth}{Xr} The test is a simple binomial test to determine whether the strategy in the rightmost 
             column is likely to have an equal number of ``wins'' as the strategy being compared against on the left. & \textbf{Test Statistics} \end{tabularx} & \textbf{p-value: 0.00534} & \textbf{Confidence Interval:  0.58234 --- 1} \\


==> table8.tex <==
-s (RecurrentConceptDriftStream -x 200000 -y 200000 -z 100 -s (generators.AgrawalGenerator -f 2 -i 2) -d (generators.AgrawalGenerator -f 3 -i 3)) & \textbf{0.11303} & 0.11828 \\
-s (RecurrentConceptDriftStream -x 200000 -y 200000 -z 100 -s (generators.RandomTreeGenerator -r 1 -i 1) -d (generators.RandomTreeGenerator -r 2 -i 2)) & \textit{\textbf{0.09855}} & \textit{\textbf{0.09855}} \\
-s (RecurrentConceptDriftStream -x 200000 -y 200000 -z 100 -s (generators.SEAGenerator -f 2 -i 2) -d (generators.SEAGenerator -f 3 -i 3)) & \textit{\textbf{0.11203}} & \textit{\textbf{0.11203}} \\
-s (RecurrentConceptDriftStream -x 200000 -y 200000 -z 100 -s (generators.STAGGERGenerator -i 2 -f 2) -d (generators.STAGGERGenerator -i 3 -f 3)) & 0.00213 & \textbf{0.00177} \\
-s (generators.HyperplaneGenerator -k 10 -t 0.0001 -i 2) & \textbf{0.10882} & 0.10884 \\
-s (generators.HyperplaneGenerator -k 10 -t 0.001 -i 2) & \textbf{0.11838} & 0.11855 \\
-s (generators.HyperplaneGenerator -k 10 -t 0.01 -i 2) & \textbf{0.11943} & 0.11982 \\
-s (generators.HyperplaneGenerator -k 5 -t 0.0001 -i 2) & \textbf{0.10675} & 0.10696 \\
-s (generators.HyperplaneGenerator -k 5 -t 0.001 -i 2) & \textbf{0.11007} & 0.11033 \\
-s (generators.HyperplaneGenerator -k 5 -t 0.01 -i 2) & \textbf{0.10528} & 0.10551 \\
-s (generators.LEDGeneratorDrift -d 1 -i 2) & \textit{\textbf{0.26121}} & \textit{\textbf{0.26121}} \\
-s (generators.LEDGeneratorDrift -d 3 -i 2) & \textit{\textbf{0.26121}} & \textit{\textbf{0.26121}} \\
-s (generators.LEDGeneratorDrift -d 5 -i 2) & \textit{\textbf{0.26121}} & \textit{\textbf{0.26121}} \\
-s (generators.LEDGeneratorDrift -d 7 -i 2) & \textit{\textbf{0.26121}} & \textit{\textbf{0.26121}} \\
-s (generators.RandomRBFGeneratorDrift -s 0.0001 -k 10 -i 2 -r 2) & \textit{\textbf{0.11975}} & \textit{\textbf{0.11975}} \\
-s (generators.RandomRBFGeneratorDrift -s 0.0001 -k 50 -i 2 -r 2) & 0.19195 & \textbf{0.19142} \\
-s (generators.RandomRBFGeneratorDrift -s 0.001 -k 10 -i 2 -r 2) & \textit{\textbf{0.15236}} & \textit{\textbf{0.15236}} \\
-s (generators.RandomRBFGeneratorDrift -s 0.001 -k 50 -i 2 -r 2) & 0.33901 & \textbf{0.3385} \\
-s (generators.WaveformGeneratorDrift -d 1 -i 2 -n) & \textbf{0.16349} & 0.16367 \\
-s (generators.WaveformGeneratorDrift -d 3 -i 2 -n) & \textbf{0.16349} & 0.16367 \\
-s (generators.WaveformGeneratorDrift -d 5 -i 2 -n) & \textbf{0.16349} & 0.16367 \\
-s (generators.WaveformGeneratorDrift -d 7 -i 2 -n) & \textbf{0.16349} & 0.16367 \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 2 -n 2 -v 2 -r 2 -b 200000 -d Recurrent) & \textbf{0.00087} & 0.00093 \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 2 -v 2 -r 2 -b 200000 -d Recurrent) & \textbf{0.00083} & 0.00097 \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 3 -v 2 -r 2 -b 200000 -d Recurrent) & 0.00161 & \textbf{0.00152} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 3 -v 3 -r 2 -b 200000 -d Recurrent) & \textbf{0.00412} & 0.00416 \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 3 -v 4 -r 2 -b 200000 -d Recurrent) & 0.01182 & \textbf{0.0117} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 3 -v 5 -r 2 -b 200000 -d Recurrent) & \textbf{0.0164} & 0.01642 \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 4 -n 2 -v 2 -r 2 -b 200000 -d Recurrent) & \textit{\textbf{0.00101}} & \textit{\textbf{0.00101}} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 4 -n 4 -v 4 -r 2 -b 200000 -d Recurrent) & \textit{\textbf{0.06557}} & \textit{\textbf{0.06557}} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 5 -n 2 -v 2 -r 2 -b 200000 -d Recurrent) & 0.00104 & \textbf{0.00101} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 5 -n 5 -v 5 -r 2 -b 200000 -d Recurrent) & \textit{\textbf{0.34081}} & \textit{\textbf{0.34081}} \\
\bottomrule &  &  \\
\begin{tabularx}{\linewidth}{Xr}
		A \textbf{bold} value indicates higher accuracy, and \textit{\textbf{bold italics}} indicate a tie.  & \textbf{Unique Wins}
		\end{tabularx} & \textbf{15} & \textbf{6} \\
\cmidrule[0.4pt](lr){2-3} &  &  \\
\begin{tabularx}{\linewidth}{Xr} The test is a simple binomial test to determine whether the strategy in the rightmost 
             column is likely to have an equal number of ``wins'' as the strategy being compared against on the left. & \textbf{Test Statistics} \end{tabularx} & \textbf{p-value: 0.9867} & \textbf{Confidence Interval:  0.13245 --- 1} \\


==> table9.tex <==
-s (RecurrentConceptDriftStream -x 200000 -y 200000 -z 100 -s (generators.AgrawalGenerator -f 2 -i 2) -d (generators.AgrawalGenerator -f 3 -i 3)) & 0.11303 & \textbf{0.11167} \\
-s (RecurrentConceptDriftStream -x 200000 -y 200000 -z 100 -s (generators.RandomTreeGenerator -r 1 -i 1) -d (generators.RandomTreeGenerator -r 2 -i 2)) & \textbf{0.09855} & 0.1128 \\
-s (RecurrentConceptDriftStream -x 200000 -y 200000 -z 100 -s (generators.SEAGenerator -f 2 -i 2) -d (generators.SEAGenerator -f 3 -i 3)) & \textbf{0.11203} & 0.11727 \\
-s (RecurrentConceptDriftStream -x 200000 -y 200000 -z 100 -s (generators.STAGGERGenerator -i 2 -f 2) -d (generators.STAGGERGenerator -i 3 -f 3)) & 0.00213 & \textbf{0.00211} \\
-s (generators.HyperplaneGenerator -k 10 -t 0.0001 -i 2) & \textbf{0.10882} & 0.11003 \\
-s (generators.HyperplaneGenerator -k 10 -t 0.001 -i 2) & 0.11838 & \textbf{0.11828} \\
-s (generators.HyperplaneGenerator -k 10 -t 0.01 -i 2) & 0.11943 & \textbf{0.11889} \\
-s (generators.HyperplaneGenerator -k 5 -t 0.0001 -i 2) & \textbf{0.10675} & 0.10986 \\
-s (generators.HyperplaneGenerator -k 5 -t 0.001 -i 2) & 0.11007 & \textbf{0.11003} \\
-s (generators.HyperplaneGenerator -k 5 -t 0.01 -i 2) & 0.10528 & \textbf{0.10476} \\
-s (generators.LEDGeneratorDrift -d 1 -i 2) & \textbf{0.26121} & 0.26129 \\
-s (generators.LEDGeneratorDrift -d 3 -i 2) & \textbf{0.26121} & 0.26129 \\
-s (generators.LEDGeneratorDrift -d 5 -i 2) & \textbf{0.26121} & 0.26129 \\
-s (generators.LEDGeneratorDrift -d 7 -i 2) & \textbf{0.26121} & 0.26129 \\
-s (generators.RandomRBFGeneratorDrift -s 0.0001 -k 10 -i 2 -r 2) & \textbf{0.11975} & 0.12437 \\
-s (generators.RandomRBFGeneratorDrift -s 0.0001 -k 50 -i 2 -r 2) & 0.19195 & \textbf{0.19145} \\
-s (generators.RandomRBFGeneratorDrift -s 0.001 -k 10 -i 2 -r 2) & \textbf{0.15236} & 0.15928 \\
-s (generators.RandomRBFGeneratorDrift -s 0.001 -k 50 -i 2 -r 2) & 0.33901 & \textbf{0.33875} \\
-s (generators.WaveformGeneratorDrift -d 1 -i 2 -n) & \textbf{0.16349} & 0.17113 \\
-s (generators.WaveformGeneratorDrift -d 3 -i 2 -n) & \textbf{0.16349} & 0.17113 \\
-s (generators.WaveformGeneratorDrift -d 5 -i 2 -n) & \textbf{0.16349} & 0.17113 \\
-s (generators.WaveformGeneratorDrift -d 7 -i 2 -n) & \textbf{0.16349} & 0.17113 \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 2 -n 2 -v 2 -r 2 -b 200000 -d Recurrent) & 0.00087 & \textbf{0.00085} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 2 -v 2 -r 2 -b 200000 -d Recurrent) & \textbf{0.00083} & 0.00084 \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 3 -v 2 -r 2 -b 200000 -d Recurrent) & \textbf{0.00161} & 0.00164 \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 3 -v 3 -r 2 -b 200000 -d Recurrent) & 0.00412 & \textbf{0.00405} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 3 -v 4 -r 2 -b 200000 -d Recurrent) & \textbf{0.01182} & 0.01201 \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 3 -n 3 -v 5 -r 2 -b 200000 -d Recurrent) & \textbf{0.0164} & 0.01832 \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 4 -n 2 -v 2 -r 2 -b 200000 -d Recurrent) & 0.00101 & \textbf{0.00098} \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 4 -n 4 -v 4 -r 2 -b 200000 -d Recurrent) & \textbf{0.06557} & 0.0675 \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 5 -n 2 -v 2 -r 2 -b 200000 -d Recurrent) & \textbf{0.00104} & 0.00106 \\
-s (generators.monash.AbruptDriftGenerator -c  -o 1.0 -z 5 -n 5 -v 5 -r 2 -b 200000 -d Recurrent) & \textbf{0.34081} & 0.34213 \\
\bottomrule &  &  \\
\begin{tabularx}{\linewidth}{Xr}
		A \textbf{bold} value indicates higher accuracy, and \textit{\textbf{bold italics}} indicate a tie.  & \textbf{Unique Wins}
		\end{tabularx} & \textbf{21} & \textbf{11} \\
\cmidrule[0.4pt](lr){2-3} &  &  \\
\begin{tabularx}{\linewidth}{Xr} The test is a simple binomial test to determine whether the strategy in the rightmost 
             column is likely to have an equal number of ``wins'' as the strategy being compared against on the left. & \textbf{Test Statistics} \end{tabularx} & \textbf{p-value: 0.97495} & \textbf{Confidence Interval:  0.20618 --- 1} \\

